Image Restoration Models with Optimal Transport and Total Variation Regularization

In this paper, we propose image restoration models using optimal transport (OT) and total variation regularization. We present theoretical results of the proposed models based on the relations between the dual Lipschitz norm from OT and the G-norm introduced by Yves Meyer. We design a numerical method based on the Primal-Dual Hybrid Gradient (PDHG) algorithm for the Wasserstain distance and the augmented Lagrangian method (ALM) for the total variation, and the convergence analysis of the proposed numerical method is established. We also consider replacing the total variation in our model by one of its modifications developed in \cite{zhu}, with the aim of suppressing the stair-casing effect and preserving image contrasts. Numerical experiments demonstrate the features of the proposed models.

==> KR_denoising/Article/KR-TV/PD.tex <==
\subsection{Primal Dual Algorithm}\label{PD-KR}
The paper \cite{2014Imaging} proposes that the original KR-TV denoising model (\ref{pro}), i.e, $K=I$, is reformulated as a convex-concave saddle point problems, 
\begin{eqnarray*}
    & \min_{u,v} \lambda_1 \|K u - f + \mathrm{div} v\|_{L_1} + \lambda_2\|v\|_{L_1} + \beta \mathrm{TV}(u) \\ 
    & = \min_{u,v} \max_{f,\phi} \int_{\Omega} (K u - f + \mathrm{div} v )\phi dx + \lambda_2\|v\|_{L_1} - I_{|\phi|_\infty\leq \lambda_1} + \int_{\Omega} \beta \nabla u \cdot v dx - I_{|v|_\infty\leq 1} .
\end{eqnarray*} 
which can be solved by the inertial forward-backward primal-dual method, with a constant inertial parameter $\alpha$.

%The above saddle-point problem can be written as
%\begin{equation}\label{PDpro}
%    \min_{u}\max_{\phi} \langle \mathcal{A} u,\phi\rangle + G(u) - F^*(\phi),
%\end{equation}
%which is a primal dual fomulation of $\min_{u} G(u) + F(\mathcal{A})$, where $\mathcal{A} = \beta \nabla, F(\phi) = \|\phi\|_2$ and $F^*(\phi) = I_{|\phi|_{\infty}\leq 1},\;, \mathcal{A}^*=-\beta \mathrm{div}$. $G(u)$ is the cascading formulation (\ref{KR-dual}),
%\begin{equation}
%    \begin{split}
%        G(u) = \min_{v} \max_{f,\phi} \int_{\Omega} (u - f + \mathrm{div} v )f dx + \lambda_2\|v\|_2 - I_{|f|_\infty\leq \lambda_1}, 
%    \end{split}
%\end{equation}

%The iteration updates of Primal Dual algorithm is
%\begin{align}
%    & \phi^{n+1} = (I+\sigma \partial F^*)^{-1}(\hat{p}) \Longleftrightarrow  \phi^{n+1}_{i,j} = \frac{\hat{p}_{i,j}}{\max\{1,|\hat{p}_{i,j}|\}}, \hat{p} = \phi^n + \sigma \mathcal{A} \bar{u}^n,\label{pd-sub1}\\
%    & u^{n+1} = (I+\tau \partial G)^{-1} (\hat{q}) = \mathrm{argmin}_{z}\{\frac{1}{2\tau} \|\hat{q}-z\|^2 + G(z)\},\hat{q} = u^n - \tau \mathcal{A}^* \phi^{n+1},\label{pd-sub2}\\
%    & \bar{u}^{n+1} = u^{n+1} + \theta(u^{n+1} - u^{n}).
%\end{align}
%We propose that the second subproblem (\ref{pd-sub2}) is solved by iterative algorithm same as (\ref{zpro}), the PD algorithm is more stable. 

%According to Theorem 1 in \cite{2011A}, the above iteration will convergence if $G(u)$ is convex, and $\tau \sigma L^2 < 1, \theta = 1$ where $L^2 = \beta^2 \|\nabla\|^2 = 8 \beta^2 / h^2$.

When $K$ is the convolution kernel, since $\int_{\Omega} (Ku) f dx = \int_{\Omega} u (K^*f) dx$, the iteration updates of Primal Dual algorithm is
\begin{equation}\label{pdhg}
    \begin{split}
        & \bar{u}^k = u^k + \alpha(u^k - u^{k-1}),\\
        & \bar{m}^k = m^k + \alpha(m^k - m^{k-1}),\\
        & \bar{v}^k = v^k + \alpha(v^k - v^{k-1}),\\
        & \bar{\phi}^k = \phi^k + \alpha(\phi^k - \phi^{k-1}),\\
        & u^{k+1} = \bar{u}^k - \mu (-\mathrm{div} \bar{v}^k + K^* \bar{f}^k)\\
        & m^{k+1} = \mathrm{shrink} (m^k + \nabla \phi^k, \mu \lambda_2), \\
        %& \hat{m}^{k+1} = 2 m^{k+1} - \bar{m}^k, \hat{u}^{k+1} = 2 u^{k+1} - \bar{u}^k, \\
        & v^{k+1} = \bar{v}^k + \beta \tau \nabla (2 u^{k+1} - \bar{u}^k), v^{k+1} = \frac{v^{k+1}}{\max\{1, |v^{k+1}|\}}\\
        & \phi^{k+1} = \phi^k + \tau (\mathrm{div} (2 m^{k+1} - \bar{m}^k) + K(2 u^{k+1} - \bar{u}^k) - u_0), \phi^{k+1} = \frac{\phi^{k+1}}{\max\{1, |\phi^{k+1}|/\lambda_1\}}.     
    \end{split}
\end{equation}
with $\mu$ and $\tau$ such that $\mu \tau \leq 1/(\|\nabla\|^2 + 2)$, and some $\alpha \in [0,1/3)$

==> KR_denoising/Article/KR-TV/Theorem_OT.tex <==
\subsection{The existence and uniqueness of minimizers of \eqref{Reg} }
If $\alpha \to 0$, the proposed model \eqref{kr_new_rel} recover the exact minimization problems \eqref{Reg}, 
\begin{equation}
    \min_u \mathcal{J}(u)=\frac{\alpha}{2} W_p(u, f)^2 + E(u),
\end{equation}
where $f \in \mathbb{P}(X)$ is a probability measure such that $\int_{\Omega} f dx = 1$.
The existence and uniqueness of minimizers of \eqref{Reg} is proved in \cite{2012Regularized} and we quote a lemma from \cite{2012Regularized}.

\begin{lemma}[cf. Burger, Martin \& Franek, Marzena \& Sch{\"o}nlieb, Carola-Bibiane \cite{2012Regularized}]
    The functional $\mathcal{J}$ has a minimizer $u \in \mathbb{P}(X)$.
\end{lemma}



\begin{lemma}[cf. Burger, Martin \& Franek, Marzena \& Sch{\"o}nlieb, Carola-Bibiane \cite{2012Regularized}]\label{exi_OT}
    Let $E$ be differentiable and strictly convex and let $\alpha>0$. Then there exists at most one minimizer of \eqref{Reg}.
\end{lemma}

\begin{proof}
    In order to prove uniqueness of a minimizer of \eqref{Wasserstein}, we use the primal and dual formulation of the Wasserstein distance.
    Assume $\int_{\Omega} u(x) dx = \int_{\Omega} f(x) dx$, denote $c(x,y)=\|x-y\|^p,p=1,2$, using the Kantorovich formulation \eqref{Kan} in problem \eqref{Reg}, it reads
    \begin{equation}\label{Wasserstein}
        \inf_{\gamma \in \mathcal{U}(\mu, \nu)}  \int_{\Omega \times \Omega} c(x,y) d \gamma(x,y) + 2\alpha E(u),
    \end{equation} 
    where $\gamma$ is the transport plan in the set
    \begin{equation}
        \left\{ \gamma \in \mathrm{Prob}(\Omega \times \Omega) :  \int_{A \times \Omega} d\gamma(x,y) = \int_{A} u(x) dx, 
        \int_{\Omega \times A} d\gamma(x,y) = \int_{A} f(y) dy,\forall A \in \Omega \right\},
    \end{equation}
    
    Using the dual formulation \eqref{kan-dual}, \eqref{Wasserstein} is written as
    \begin{eqnarray}\label{reg-dual}
    \min_{u}\max_{\phi,\psi} \left\{ 2\alpha E(u) + \int_\Omega \phi(x) u(x) dx + \int_\Omega \psi(y) f(y) dy : \psi(x) + \phi(x) \leq c(x,y) \right\}
    \end{eqnarray}

    The optimality condition for $u$ implies 
    \begin{equation}\label{opt_con}
        2\alpha \langle E'(u), u-v\rangle + \int_{\Omega} \phi(x) (u(x)-v(x)) dx \leq 0
    \end{equation}
    for all admissible density $v$.

    Assume $u_1,u_2$ are minimizer of \eqref{Wasserstein} with associated transport maps $\gamma_i,i=1,2$ and $\phi_i,\psi_i$ are the associated variables in \eqref{reg-dual}, then from \eqref{opt_con},
    \begin{equation}\label{u_i}
        2\alpha \langle E'(u_1) - E'(u_2), u_1 - u_2\rangle \leq -\int_{\Omega}(\phi_1(x)-\phi_2(x)) (u_1(x)-u_2(x)) dx,
    \end{equation}
    
    According to the primal-dual relationship in \cite{Peyr2019Computational},
    \begin{equation}\label{complementary}
        (\phi(x) + \psi(y) - c(x,y)) \gamma(x,y) = 0,\forall (x,y) \in \Omega \times \Omega,
    \end{equation}
    Using \eqref{complementary} and the definition \eqref{c-tra}, we obtain
    \begin{align*}
    & \int_{\Omega}(\phi_1(x)-\phi_2(x))(u_1(x)-u_2(x)) dx = \int_{\Omega \times \Omega} \phi_1(x) d\gamma_1(x,y) - \int_{\Omega \times \Omega} \phi_1(x) d\gamma_2(x,y)\\
    & -\int_{\Omega \times \Omega} \phi_2(x) d\gamma_1(x,y) + \int_{\Omega \times \Omega} \phi_2(x) d\gamma_2(x,y)\\
    & \geq \int_{\Omega \times \Omega} (c(x,y) - \psi_1(y)) d\gamma_1(x,y) - \int_{\Omega \times \Omega} (c(x,y) - \psi_1(y)) d\gamma_2(x,y)\\
    & -\int_{\Omega \times \Omega} (c(x,y) - \psi_2(y)) d\gamma_1(x,y) + \int_{\Omega \times \Omega} (c(x,y) - \psi_2(y)) d\gamma_2(x,y)\\
    & = \int_{\Omega \times \Omega} (\psi_2(y)-\psi_1(y)) d\gamma_1(x,y) - \int_{\Omega \times \Omega} (\psi_2(y)-\psi_1(y)) d\gamma_2(x,y)\\
    & \geq \int_{\Omega} (\psi_2(y)-\psi_1(y)) df(y) - \int_{\Omega } (\psi_2(y)-\psi_1(y)) df(y) = 0.
    \end{align*}
    Thus $-\int_{\Omega}(\phi_1(x)-\phi_2(x))(u_1(x)-u_2(x)) dx \leq 0$, and if $E$ is strictly convex, then $u_1 = u_2$.

\end{proof}




\begin{lemma}[cf. Burger, Martin \& Franek, Marzena \& Sch{\"o}nlieb, Carola-Bibiane \cite{2012Regularized}]
    Let $E$ be differentiable and strictly convex and let $\alpha>0$, and let $u_i,i=1,2$ be minimizer of \eqref{Reg} for $f_i,i=1,2$, then the symmetric Bregman distance is bounded by,
    \begin{eqnarray}
    2\alpha \langle E'(u_1) - E'(u_2), u_1 - u_2 \rangle \leq W_c(f_1,f_2).            
    \end{eqnarray}
    where $W_c(f_1,f_2) = \inf_{\gamma \in \mathcal{U}(f_1, f_2)} \int_{\Omega \times \Omega} c(x,y) d \gamma(x,y)$.
\end{lemma}

\begin{proof}
        Recall the formulation of the dual problem in terms of c–concave functions \eqref{c-tra}, the supremum in \eqref{kan-dual} can be restricted to $((\phi^{c})^c, \phi^c)$. Using \eqref{u_i} and replacing $\phi_i,\psi_i$ for $\phi_i^{cc},\phi_i^c,i=1,2$ in the proof in Theorem \ref{exi_OT}, one obtains 
    \begin{eqnarray}
        2\alpha \langle E'(u_1) - E'(u_2), u_1 - u_2 \rangle & \leq - \int_{\Omega}(\phi_1^{cc}(x)-\phi_2^{cc}(x))(u_1(x)-u_2(x)) dx \\
        & \leq \int_{\Omega} (\phi_1^c(y)-\phi_2^c(y)) d (f_1(y) - f_2(y))\\            
    \end{eqnarray}
    
    Let $c(x,y)=\|x-y\|^p,p=1,2$, the function $\phi_i^c,i=1,2$ satisfy
    \begin{eqnarray}
     \phi_i^c(y) - \phi_i^c(y') & = \inf_x\{c(x,y)-\phi_i(x)\} + \sup_x\{\phi_i(x)-c(x,y')\}\\
     & \leq \sup_x \{c(x,y) - c(x,y')\} \leq c(y,y'),
    \end{eqnarray}
    
    Let $d(x,y)=c(x,y)$ in \eqref{Lipschitz}, then $\mathrm{Lip}(\phi_i^c) \leq 1,i=1,2$,
    \begin{eqnarray}
    2\alpha \langle E'(u_1) - E'(u_2), u_1 - u_2 \rangle \leq \int_{\Omega} (\phi_1^c(y)-\phi_2^c(y)) d (f_1(y) - f_2(y))\\
    \leq \sup_{\Phi} \{ \int_{\Omega} \Phi(y) d (f_1(y) - f_2(y)) : \mathrm{Lip}(\Phi) \leq 2 \}.
    \end{eqnarray}

    According to the Proposition \ref{KR-theorem},
    \begin{equation}
        \sup_{\Phi} \{ \int_{\Omega} \Phi(y) d (f_1(y) - f_2(y)) : \mathrm{Lip}(\Phi) \leq 2 \} = 2 W_c(f_1,f_2)
    \end{equation}

    However, in the case of total variation, there exist $u_1 \neq u_2$ such that $E'(u_1) - E'(u_2)=0$.    $\hfill\square$
\end{proof}






==> KR_denoising/Article/KR-TV/Theorem_lip.tex <==
\subsection{Existence of the Solutions of the proposed model \eqref{kr_new_rel}}
The following lemmas can be proved by generalization of the mathematical results in \cite{2005Image,2006Structure} for the G-TV model. 



\begin{lemma}[cf. Jean-Fran{\c{c}}ois Aujol \& Gilles Aubert \cite{2005Image}]\label{dis-G}
The discrete version of the $G$ space \eqref{g-space} is
\begin{equation}
    G = \{v \in V : v = \mathrm{div}(g),\quad \exists g \in Q\},
\end{equation}
where $\mathrm{div}$ is the backward differences with homogeneous Dirichlet boundary conditions, then $G$ identifies with
\begin{equation}\label{g-spa-dis}
    G = \{v \in V : \sum_{i,j} v(i,j) = 0\},
\end{equation}
\end{lemma}
Lemma \ref{dis-G} means the dual Lipschitz norm \eqref{lip-dual} is well defined for $v \in G$ in discrete settings.




\begin{lemma}
   There exist a solution $(\vec{u},\vec{v})$ that minimize \eqref{kr_new_rel_dis}.
\end{lemma}
\begin{proof}
    \begin{enumerate}
        \item $F_{\alpha,\lambda}$ is convex and lower semi-continuous on $V \times V$.
        \item We want to prove that $F_{\alpha,\lambda}$ is coercive on $V \times V$. 
        By contradiction, let us assume if
        \begin{equation}\label{ass_1}
            \|(u,v)\|_V = \sqrt{\|u\|^2 + \|v\|^2} \longrightarrow \infty,
        \end{equation}
        there exist a constant $C$ such that $F_{\alpha,\lambda} < C$. 
        Then we have $\lambda \|v\|_{\mathrm{Lip}^*} I_{v \in G} < C$, thus $v \in G$ and there exists $m \in V$ such that $v = \mathrm{div}(m)$ and $\|m\|_2 = \|v\|_{\mathrm{Lip}^*} < C/\lambda$.
        By the definition of $\mathrm{div}$ \eqref{div}, we have
        \begin{equation}\label{v_inq_1}
            \|v\|_V \leq 4 \sum_{1\leq i,j\leq N} (|m(i,j,1)| + |m(i,j,2)|+|m(i-1,j,1)| + |m(i,j-1,2)|) < 4 C/\lambda.
        \end{equation}
        Moreover, since $\frac{1}{2\alpha} \|f-u-v\|^2 < C$, we get from \eqref{v_inq_1} that $\|u\|_V$ is bounded. This contradicts our assumption \eqref{ass_1}, thus we conclude $F_{\alpha,\lambda}$ is coercive on $V \times V$.
    \end{enumerate}
We deduce the existence of a minimizer $(\hat{u}, \hat{v})$.     $\hfill\square$
\end{proof}

==> KR_denoising/Article/KR-TV/shrink.tex <==
\subsubsection{"shrink" Operators}\label{sec_shrink}
The "shrink" operators for some norms $\|\cdot\|$ has closed form solutions \cite{2017Vector}
    \begin{equation}\label{shrink}
        \mathrm{shrink}(x^0; \mu) = \mathrm{argmin}_{z}\{\mu \|z\| + (1/2 \|z-x\|^2\}.
    \end{equation}
For $\mu>0$, define $\mathrm{shrink}_1: \mathbb{R} \to \mathbb{R}$ as
\begin{equation}
    \mathrm{shrink}_1(x; \mu) = \max\{1-\mu/|x|, 0\}x.
\end{equation}
Define $\mathrm{shrink}_2: \mathbb{R}^r \to \mathbb{R}^r$ as
\begin{equation}
    \mathrm{shrink}_2(x; \mu) = \max\{1-\mu/\|x\|_2, 0\} x.
\end{equation}
where $\|\cdot\|_2$ is the standard Euclidean norm.

If $x = (x_1,x_2,\cdots,x_r)$ and $\|x\|=\|x_1\|_1 + \|x_2\|_2 + \cdots + \|x_r\|_r$ for some norms $\|\cdot\|_1,\cdots,\|\cdot\|_r$, then
\begin{equation}
    \mathrm{shrink}(x;\mu) = \left[\begin{array}{c}
        \mathrm{shrink}_1(x_1;\mu) \\
        \vdots \\
        \mathrm{shrink}_r(x_r;\mu) \\
    \end{array}
    \right],
\end{equation}
where $\mathrm{shrink}_i,i=1,2,\cdots,r$ are the associated shrink operators.

==> KR_denoising/Article/Other/SISR_ALM.tex <==
Morever, the mathematical formulation of Single Image Super-Resolution (SISR) degradation model is given by
\begin{equation}\label{sisr}
    y = G * x + n = (K * x) \downarrow_s,
\end{equation}
where $k$ is a blurring operator and $\downarrow_s$ means selecting the upper-left pixel for each distinct patch of size $s \times s$ \cite{2020Plug}. (When $s=1$, it is the same as the image deblurring model.) 

For SISR modeled in (\ref{sisr}), the u-subproblem $\min_{u\in V} \mathcal{G}(u)$ can be formulated as
    \begin{equation}\label{sub-sisr}
        \hat{u} = \mathrm{argmin}_{u \in \mathbb{R}^n} \|G u - \hat{y}\|^2 + \rho \|\nabla u - \hat{z}\|^2,
    \end{equation}
    where  $\rho = r_p/r_z$, $\hat{z} = p + \lambda_p/r_p$ and $\hat{y} = z + \lambda_z/r_z$, and the optimality condition is 
    \begin{equation}\label{EL}
    (G^TG - \rho \Delta) \hat{x} = G^T y - \rho \mathrm{div} \hat{z} = b.
    \end{equation}
    According to \cite{2020Plug}, using the the Woodbury inverse formula, we have
    \begin{equation}
        (G^TG - \rho \Delta)^{-1} = -\rho^{-1}(\Delta^{-1} -  \Delta^{-1}G^T(\rho I - G\Delta^{-1}G^T)^{-1} G \Delta^{-1} ),
    \end{equation}
    then the closed-form solution of the above problem (\ref{sub-sisr}) is 
    \begin{equation}\label{fft-sisr}
        \mathcal{F}(\hat{x}) = -\rho^{-1}\mathcal{F}(\Delta^{-1})(\mathcal{F}(b) + (\mathcal{F}(k)^* \odot_s \frac{(\mathcal{F}(k) \mathcal{F}(\Delta^{-1}) \mathcal{F}(b))\Downarrow_s}{(\mathcal{F}(k)^* \mathcal{F}(\Delta^{-1}) \mathcal{F}(k))\Downarrow_s + \rho}))
    \end{equation}
    where $\odot_s$ means applying elementwise multiplication to $s \times s$ distinct blocks of $\mathcal{F}(k)^*$,
    $\Downarrow_s$ means averaging the $s \times s$ distinct blocks.


==> KR_denoising/Article/Other/TGV.tex <==
\subsection{Total Generalized Variation (TGV)}
In \cite{Bredies2010TotalGV}, a novel concept of total generalized variation (TGV) is introduced, which involves and balances higher-order derivatives of $u$ and reduces the staircasing effect.
%We can take $R(u) = \mathrm{TGV}_{\alpha}^2(u)$ which is defined as follows. 

Define $\mathrm{Sym}^2(\mathbb{R}^d) = S^{d\times d},\;d=2$ as the space corresponds to symmetric matrices.
For $v \in \mathrm{Sym}^2(\mathbb{R}^d)$,
\begin{equation}\label{TGV}
    (\mathrm{div} v)_i = \sum_{j=1}^d \frac{\partial v_{ij}}{\partial x_j}, \quad \mathrm{div}^2 v = \sum_{0<i,j\leq d} \frac{\partial^2 v_{ij}}{\partial x_i\partial x_j},
\end{equation}

The second-order total generalized variation is defined as 
\begin{equation}
    \begin{split}
        \mathrm{TGV}_{\alpha}^2(u) = \sup\{\int_{\Omega} u \mathrm{div}^2 v dx : v \in \mathcal{C}_c^2(\Omega, \mathrm{Sym}^2(\mathbb{R}^d)),\\
         \|\mathrm{div}^l v\|_{\infty} \leq \alpha_l, l=0,1\},
    \end{split}
\end{equation}



\subsubsection{Primal Dual Algorithm for TGV}

A discrete version of image denoising model with $\mathrm{TGV}_{\alpha}^2$ (\ref{TGV}) regularizer and KR norm is given by,
\begin{equation}\label{tgv}
    \min_{u \in U} \{\|f - u\|^h_{KR,\lambda} + \sup_{v} (\langle(\mathrm{div})^2 v, u\rangle\} - I_{v \in J^h}).
\end{equation}
where $J^h = \{v \in V | \|v\|_{\infty} \leq \alpha_0,\; \|\mathrm{div} v\|_{\infty} \leq \alpha_1\}$, and $\|f - u\|^h_{KR,\lambda}$ is given by (\ref{W1PD-KR}).

Let $\mathcal{A} = ((\mathrm{div})^2)^*, F^*(v) = I_{v \in J}$ and we can solve the model with total generalized variation (\ref{tgv}) using the above primal dual algorithm (\ref{PDpro}) where $L^2 = \|(\mathrm{div})^2\|^2 = (8 / h^2)^2$.

The computation of the first sub-problem (\ref{pd-sub1}) is the projection of a variable $\hat{v}$ onto the convex set $J^h$
\begin{equation}
    \Pi_{J^h} (\hat{v}) = \argmin_v \frac{ \|v - \hat{v}\|^2}{2\sigma} + I_{J^h}(\Gamma v),
\end{equation}

The author adopt the fast shrinkage thresholding algorithm (FISTA) for this problem, and run the iterative projection algorithm until the maximal feasibility error of $\Pi_{K^h} (\hat{v}^h)$ is below a threshold $\epsilon$ for each outer iteration \cite{Bredies2010TotalGV}, which is similar to our algorithm since we take inner iterations (\ref{pdhg}) as well.

==> KR_denoising/Article/Other/Theorem.tex <==
\section{Convergence Analysis of ALM}\label{Theorem}
%\subsection{Properties of KR-TV Denoising}
We quote two lemmas from \cite{2014Imaging} for completeness.

\begin{theorem}\label{mass}
    (Mass preservation) If $\frac{\lambda_2}{\lambda_1} \leq \frac{2}{\mathrm{diam}(\Omega)}$, then
    (\ref{pro}) has a minimizer $\hat{u}$ such that $\int_\Omega \hat{u}(x) dx = \int_\Omega u^0(x) dx$.
    It holds that a minimizer of the KR-TV denoising problem
    with $\lambda_1 = \infty$ is also a minimizer of the problem when $\lambda_1 > \frac{\lambda_2 \mathrm{diam}(\Omega)}{2}$.
\end{theorem}
 
\begin{theorem}\label{KR-dual}
    (Cascading formulation) Let $\Omega$ be open, convex, and bounded, and let $\lambda = (\lambda_1,\lambda_2) \geq 0$. The dual formulation of (\ref{KR-norm}) is 
\begin{equation}
    \begin{split}
        \|\mu\|_{KR,\lambda} & = \min_{\vec{v} \in \mathcal{R}(\bar{\Omega},\mathbb{R}^2)}  \lambda_1 \|\mu + \mathrm{div} \vec{v}\|_{\mathcal{R}} + \lambda_2\||\vec{v}|\|_{\mathcal{R}}\\
        & = \int_\Omega \phi(\mu + \mathrm{div} \vec{v})dx - I_{|\cdot|_{\infty}\leq \lambda_1}(\phi) + \lambda_2\||\vec{v}|\|_{\mathcal{R}}
    \end{split}
\end{equation}
    where $\|\vec{v}\|_{\mathcal{R}} = \sup_{|\vec{f}|\leq 1} \int_\Omega \vec{f} d \vec{v}$, $\mathrm{div} \vec{v}$ is taken in $\bar{\Omega}$ or any open set $U$ containing $\bar{\Omega}$.
\end{theorem}

%\subsection{Convergence analysis }

\begin{theorem}
    Suppose $(u^*, p^*, z^*, \lambda_p^*, \lambda_z^*)$ is saddle point of the $\mathcal{L}(u,p,z,\lambda_p,\lambda_z)$ and assume  $R(u) = \mathrm{TV}(u)$ in (\ref{lag}) and $\lambda_1 = \infty$.
    Let $(u^{\ell}, p^{\ell}, z^{\ell}, \lambda_p^{\ell}, \lambda_z^{\ell})$ be the sequence generated by Algorithm \ref{alg1},
    then in the discrete setting, we have
    \begin{equation}
        \lim \limits_{\ell\to +\infty} \|z^{\ell} - Ku^{\ell}\| = 0.
    \end{equation}
\end{theorem}


Since the proof is similar to Theorem 4.3 in \cite{2017Augmented}, we only provide a sketch of the proof and points out the difference.
The only difference between our model and that in \cite{2017Augmented} is the definition of $F(z)$ and mesh size $h$, we can take $h=1$ and $\lambda_1 = \infty$,
\begin{equation}\label{fz}
    F(z) = \|z-f\|_{KR,\lambda} = \min_{m} \max_{\phi} \langle z - f + \mathrm{div} m ,\phi \rangle + \lambda_2\|m\|_2 - I_{|\phi|_{\infty}\leq \lambda_1},
\end{equation}
    For given $(\lambda_z,u)$, the discretization of $\mathcal{G}(z)$ (\ref{zpro}) is written as
    \begin{equation}\label{saddle}
        \mathcal{L}(z,m,\phi,\lambda_z,u) = \min_z \min_{m} \max_{\phi} (\langle z - f + \mathrm{div} m, \phi \rangle + \lambda_2\|m\|_2 - I_{|\phi|_{\infty}\leq \lambda_1} + \langle \lambda_z, z\rangle + \frac{r_z}{2}\|z - Ku\|^2) h^2.
    \end{equation}
    
%So the equation (40) and (43) in\cite{2017Augmented}, i.e, the following two equation, have to be proven.
    %Since $p^* = \mathrm{argmin}_p \mathcal{L}(u^*, p^*, z^*, \lambda_p^*, \lambda_z^*)$, then for funtion $y(t) = \mathcal{L}(u^*, p^* + t(p - p^*), z^*, \lambda_p^*, \lambda_z^*)$, for any $p$ and $t\in[0,1]$, we have $y'(0) \geq 0$.
    %thus
    %\begin{equation}
    %    (\nabla_p \mathcal{L}|_{p=p^*},p-p^*) =  (\nabla_p\phi_a (|p^*|) + \gamma_1(p^*-\nabla u^*) + \lambda_1^*, p-p^*) \geq 0, \forall p.
    %\end{equation}
    %since $h(x) = \phi_a (|x|) + \frac{\gamma}{2}(x-\nabla u^*)^2 $ is convex when $\gamma > \frac{1}{a}$,
    %\begin{equation}
    %    F(z) - F(z^*) + \langle \lambda_z^*, z-z^*\rangle + r_z\langle z^* - Ku^*, z-z^* \rangle \geq 0, z = z^{\ell},
    %\end{equation} 
    %\begin{equation}
    %    F(z) - F(z^{\ell}) + \langle \lambda_z^{\ell}, z-z^{\ell}\rangle + r_z\langle z^{\ell} - Ku^{\ell}, z-z^{\ell}\rangle \geq 0, z = z^*,
    %\end{equation} 


    Since $z^* = \mathrm{argmin}_z \mathcal{L}(u^*, p^*, z, \lambda_p^*, \lambda_z^*)$,
    then for the funtion $y(t) = \mathcal{L}(u^*, p^*, z^* + t(z - z^*), \lambda_p^*, \lambda_z^*)$, for any $z$ and $t\in[0,1]$, we have $y'(0) \geq 0$,
    and thus
    \begin{equation}\label{eqz1}
        \langle \nabla_z F(z^*) + \lambda_z^* + r_z (z^*- Ku^*) , z - z^* \rangle \geq 0, \forall z,
    \end{equation}
    Similarly, since $z^{\ell} = \mathrm{argmin}_z \mathcal{L}(u^{\ell}, p^{\ell}, z, \lambda_p^{\ell}, \lambda_z^{\ell})$, we have
    \begin{equation}\label{eqz2}
        \langle \nabla_z F(z^{\ell}) + \lambda_z^{\ell-1} + r_z (z^{\ell}- Ku^{\ell}) , z - z^{\ell}\rangle \geq 0, \forall z,
    \end{equation}

    Similar to \cite{2017Augmented}, the following equation holds,
    \begin{eqnarray}
        & R(p) - R(p^*) + \langle\lambda_p^*, p-p^*\rangle + \langle p^* - \nabla u^*, p-p^*\rangle \leq 0,\forall p \in Q,\label{eqp1}\\
        & R(p) - R(p^{\ell}) + \langle\lambda_p^{\ell}, p-p^{\ell}\rangle + \langle p^{\ell} - \nabla u^{\ell}, p-p^{\ell}\rangle \leq 0,\forall p \in Q,\label{eqp2}
    \end{eqnarray}

\begin{equation}
\begin{split}
 \langle \mathrm{div} \lambda_p^*, u-u^*\rangle + r_p\langle \mathrm{div} (p^*-\nabla u), u-u^*\rangle + \langle \lambda_z^*, -K(u-u^*)\rangle\\
        + r_z\langle z^*-Ku^*, -K(u-u^*)\rangle \geq 0, \forall z\in V, \label{equ1}
\end{split}
\end{equation}  

\begin{equation}
\begin{split}
 \langle \mathrm{div} \lambda_p^{\ell}, u-u^{\ell}\rangle + r_p\langle \mathrm{div} (p^{\ell}-\nabla u), u-u^{\ell}\rangle + \langle \lambda_z^{\ell}, -K(u-u^{\ell})\rangle\\
        + r_z\langle z^{\ell}-Ku^{\ell}, -K(u-u^{\ell})\rangle \geq 0, \forall z\in V,\label{equ2}
  \end{split}
\end{equation}  


    Taking $z = z^{\ell}$ in (\ref{eqz1}), $z = z^*$ in (\ref{eqz2}), $p = p^{\ell}$ in (\ref{eqp1}), $p = p^*$ in (\ref{eqp2}), $u = u^{\ell}$ in (\ref{equ1}), $u = u^*$ in (\ref{equ2}), respectively, and add the equations, we have
    \begin{eqnarray*}
        & - \bar{\lambda_p}^{\ell}(\bar{p}^{\ell} - \nabla \bar{u}^{\ell}) - \bar{\lambda_z}^{\ell}(\bar{z}^{\ell} - K*\bar{u}^{\ell}) \geq r_p \|\bar{p}^{\ell} - \nabla \bar{u}^{\ell}\|^2 + r_z \|\bar{z}^{\ell} - K*\bar{u}^{\ell}\|^2 \\
        & + r_p \langle \nabla \bar{u}^{\ell}, \bar{p}^{\ell} - \bar{p}^{\ell-1}\rangle + r_z \langle K*\bar{u}^{\ell}, \bar{z}^{\ell} - \bar{z}^{\ell-1}\rangle \\
        & + \langle z^{\ell} - z^*, \nabla F(z^{\ell}) - \nabla F(z^*)\rangle ,
    \end{eqnarray*}
    where $\bar{z}^{\ell} = z^{\ell} - z^*, \bar{p}^{\ell} = p^{\ell} - p^*,\bar{u}^{\ell} = u^{\ell} - u^*, \bar{\lambda_z}^{\ell} = \lambda_z^{\ell} - \lambda_z^*,\bar{\lambda_p}^{\ell} = \lambda_p^{\ell} - \lambda_p^*$.

    If $\langle z^{\ell}-z^*, \nabla F(z^{\ell}) - \nabla F(z^*)\rangle \geq 0$ hold, then (44) in \cite{2017Augmented} is proved and the rest of proof is the same.

    When $\lambda_1 = \infty$, suppose the $(z^k,m^k,\phi^k)$ in algorithm (\ref{pdhg}) converges to $(\hat{z},\hat{m},\hat{\phi})$ which is a saddle points of (\ref{saddle}), then $ \hat{z} - f + \mathrm{div} \hat{m} = 0$, and $\sum_{i=1}^N\sum_{j=1}^M\hat{z} = \sum_{i=1}^N\sum_{j=1}^M f$.
    
    %Since $z^{\ell}$ and $z^*$ are saddle points of $\mathcal{G}(z)$ (\ref{zpro}) for given $(\lambda_z^{\ell-1},u^{\ell})$ and $(\lambda_z^*,u^*)$, $\|z^{\ell}\|_1 = \|z^*\|_1 = \|f\|_1$ holds.



\begin{theorem}
    If $\lambda_1 = \infty$, $F(z)$ (\ref{fz}) is convex in $D = \{z: \sum_{i=1}^N\sum_{j=1}^M z = \sum_{i=1}^N\sum_{j=1}^M f\}$, i.e., for $z^{\ell},z^j\in D$,
    we have \begin{equation}
        \langle z^{\ell}-z^j, \nabla F(z^{\ell}) - \nabla F(z^j)\rangle \geq 0.
    \end{equation}
\end{theorem}

    The proof for the above inequality is similar to Theorem 1 in \cite{2016A}.  
    For $\hat{z}\in D$, there exist $(\hat{m},\hat{\phi})$ which is a saddle points
    \begin{equation}
        F(z) = \|z-f\|_{KR,\lambda} = \min_{m} \max_{\phi} \langle z - f + \mathrm{div} m ,\phi \rangle + \lambda_2\|m\|_2,
    \end{equation}
    %$(z^{\ell},m^{\ell},\phi^{\ell})$ is a saddle point of $L(z,m,\phi,\lambda_z^{\ell-1},u^{\ell})$ (\ref{saddle}).
    %Similarly, there exists $(m^j,\phi^j)$ such that $(z^j,m^j,\phi^j)$ is a saddle points of $L(z,m,\phi,\lambda_z^{j-1},u^j)$.
    then the optimality condition gives,
    \begin{equation}\label{opt}
        \begin{split}
            & 0 = \frac{\partial L}{\partial m}|_{\hat{z},\hat{m},\hat{\phi}} = \lambda_2 \frac{\partial \|\hat{m}\|_2}{\partial \hat{m}} - \nabla \hat{\phi} ,\\
            & 0 = \frac{\partial L}{\partial \phi}|_{\hat{z},\hat{m},\hat{\phi}} = \hat{z} - f + \mathrm{div} \hat{m},                
        \end{split}
    \end{equation}
    Thus 
    \begin{equation}
        \|\nabla \hat{\phi}\|_p = \lambda_2 \|\frac{\hat{m}}{\|\hat{m}\|_2}\|_2 = \lambda_2,\; \|\hat{m}\|_2 \geq 0,
    \end{equation}

    By the construction of $z^{\ell},z^j$, there exist $(m^{\ell},\phi^{\ell})$ and $(m^j,\phi^j)$ satisfies the optimality condition (\ref{opt}), respectively. 
    Since $\nabla_{z} F(z^{\ell}) = \phi^{\ell}$ and $\nabla_{z} F(z^*) = \phi^*$, we have
    \begin{align}
        & \langle z^{\ell}-z^j, \nabla_z F(z^{\ell}) - \nabla_z F(z^j)\rangle = \langle z^{\ell}-z^j, \phi^{\ell}-\phi^j \rangle = \langle \phi^{\ell}-\phi^j, \mathrm{div} m^j - \mathrm{div} m^{\ell}\rangle\\
        & = \langle \nabla \phi^{\ell} - \nabla \phi^j, m^{\ell} - m^j\rangle = \langle\frac{ \partial \|m^{\ell}\|_2}{\partial m}-\frac{ \partial \|m^j\|_2}{\partial m}, m^{\ell} - m^j\rangle \geq 0.
    \end{align}
    The last inequality holds is due to $\|m\|_2$ is convex.

 



%By $p^k = \mathrm{argmin}_p \mathcal{L}(u^k,p,z^{k-1},\lambda_1^{k-1},\lambda_2^{k-1})$ and $p^{k-1} = \mathrm{argmin}_p \mathcal{L}(u^{k-1},p,z^{k-2},\lambda_1^{k-2},\lambda_2^{k-2})$,
%\begin{equation}
%    <p^{k-1} - p^k, \lambda_1^{k-1} - \lambda_1^k> = <p^{k-1} - p^k, \gamma_1(\nabla u^k - dp^k)> \leq 0.
%\end{equation}

%with (46) in \cite{2017Augmented}, the proof is completed. 



==> KR_denoising/Article/Other/W1.tex <==
%According to the theory of optimal transport \cite{Peyr2019Computational}, 
According to the theory of optimal transport \cite{Peyr2019Computational}, the global Lipschitz constraint in (\ref{KR}) can also be made as a a uniform bound on the gradient of $\phi$. 
The computation of $W_1(u, \nu)$ is equivalent to a new minimization problem, 
\begin{equation}\label{W1}
    \begin{split}
        &\max_{\phi:\Omega \longrightarrow \mathbf{R}}\,\, \int_{x \in \Omega} \phi(x)(u(x) - \nu(x)) dx \\
        &s.t.\quad
            \|\nabla \phi(x)\|_2 \leq 1, a.e.x\in \Omega,   
    \end{split}
\end{equation}
and the dual problem of (\ref{W1}) is
\begin{equation}\label{W1-dual}
    \begin{split}
    & \min_{m:\Omega \longrightarrow \mathbf{R}^2}\,\, \int_{x \in \Omega} \|m(x)\|_2 dx \\
    & s.t.\quad
        \mathrm{div}(m(x)) = u(x) - \nu(x),\; \forall x \in \Omega,\\
    &	m(x) \cdot n(x) = 0, \forall x \in \partial \Omega,
    \end{split}
\end{equation}

%When $(\lambda_1,\lambda_2) = (\infty,1)$, KR norm (\ref{KR-norm}) recovers (\ref{KR}) which is the same as Wasserstein-1 metric (\ref{W1}), i.e.,$ \|u-f\|_{KR,\infty,1} = W_1(u,f)$. And the dual formulation of KR norm (\ref{KR-dual}) is the same as (\ref{W1-dual}) by letting $\mu = \rho^1(x) - \rho^0(x)$.
%Therefore we can compute the KR norm (\ref{KR-norm}) using the same discretization and algorithms for Wasserstein-1 metric as follows.

%The definition of KR norm (\ref{KR-norm}) only differs the Wasserstein-1 distance (\ref{W1}) in the parameters $\lambda_1,\lambda_2$. 


%Note that the discretization of the dual formulation of KR norm $\|u-f\|_{KR,\lambda}$ (\ref{KR-dual})
%\begin{equation}\label{W1PD-KR}
%    \|u-f\|_{KR,\lambda}^h = \min_{m}\max_{\phi} \langle u - f + \mathrm{div} m ,\phi \rangle - I_{|\phi|_\infty\leq \lambda_1} + \lambda_2\|m\|_2
%\end{equation}
%is exactly the same as (\ref{W1PD}) besides parameters $\lambda_1,\lambda_2$, we can compute it using the same algorithm as (\ref{W1PD}).

%and the discretization of the KR-TV model (\ref{pro}) is
%\begin{equation}
%    \min_{u_h, m_h}\max_{\phi_h} h^2 (\langle u - f + \mathrm{div}_h m_h ,\phi_h \rangle - I_{|\phi|_\infty\leq \lambda_1} + \lambda_2\|m_h\|_2 + \beta R(\nabla_h u_h)).
%\end{equation} 

%The discretized version of problems (\ref{W1}) and (\ref{W1-dual}) can be jointly solved by the following Lagrangian function, 
%\begin{equation}\label{W1PD}
%    \min_{m} \max_{\phi} L(m, \phi) = \|m\|_2 + \langle \phi, \mathrm{div} (m) - u + \nu \rangle, 
%\end{equation}
%the saddle point of which can be computed with the first-order primal-dual method of Chambolle and Pock \cite{2011A}.

==> KR_denoising/Article/Other/siam_car_tex.tex <==
\section{$u+v+w$ Image Restoration Model}
%The degradation model is 
%\begin{equation}
%    f = K(u+v) + n
%\end{equation}
%where $K$ is a convolution operator, and $n$ is the noise. In the purely denoising model, $K=I$ where $I$ is an identity matrix.
%The aim is to recover an image $\hat{u} = u+v$ and decompose $\hat{u}$ into cartoon and texture components, denoted by $u$ and $v$.

%In this paper, we propose an image restoration model with the dual Lipschitz norm,
%\begin{equation}\label{KV-lip}
%    \inf_{(u,v)\in BV\times H} \int_{\Omega} R(|\nabla u|) + \frac{\alpha}{2} \int_{\Omega} |f-K(u+\Delta g)|^2 dx + \lambda \lambda \||\nabla g|\|_{L^1}.
%\end{equation}









%Note that the component $v = \mathrm{div}(m)$ in \eqref{kr_new_rel}, while in \eqref{KV-lip} the component $v$ is modeled as $\Delta g$, where $\nabla g = m$. 




%If there is no noise in the image, the parameter $\alpha$ is large to ensure $r = f-K*(u+\Delta g) \approx 0$, and if the variance of the additive noise is $\sigma^2$, then $\alpha$ is chosen so that the constraint $\|f-K*(u+\Delta g)\|^2_{L^2} \approx \sigma^2$.

\subsubsection{ADMM Algorithm}\label{admm}
In \cite{doi:10.1137/140967416}, the authors applied the
ADMM algorithm to solve the model \eqref{KV-Jung}.
The ADMM algorithm is often applied to solve constrained optimizations with linear equality constraints
\begin{equation}
    \min\{\theta_1(x)+\theta_2(x) : Ax+By=b, x \in \mathbb{R}^{d\times m_1}, y \in \mathbb{R}^{d\times m_2}\}
\end{equation}
Its Lagrange function is 
\begin{eqnarray}
    L(x,y,\lambda) = \theta_1(x)+\theta_2(x) - \lambda^T(Ax+By-b).
\end{eqnarray}
apply the ALM to it, the $k$-th iteration
\begin{eqnarray}
    & x^{k+1} = \mathrm{arg}\min_x \{ L(x,y^k,\lambda^k) + \frac{\beta}{2}\|Ax+By^k-b\|^2\},\\
    & y^{k+1} = \mathrm{arg}\min_y \{ L(x^{k+1},y,\lambda^k) + \frac{\beta}{2}\|Ax^{k+1}+By-b\|^2\},\\
    & \lambda^{k+1} = \lambda^k - \beta(Ax^{k+1}+By^{k+1}-b).
\end{eqnarray}

\input{KR_denoising/Article/KR-TV/Discretization_ALM}

The unconstrained problem \eqref{KV-Jung} can be converted model to its constrained form
\begin{equation}
    \begin{split}
        & \inf_{u,g} \int_{\Omega} R(|d_2|) + \frac{\alpha}{2} \int_{\Omega} |f-K(u+\Delta g)|^2 dx + \lambda \||d_1|\|_{L^1},\\
        & s.t.\quad g = z, \quad d_1 = \nabla z, \quad d_2 = \nabla g.
    \end{split}
\end{equation}
The authors apply the ADMM algorithm to the constrained model.

The augmented Lagrangian functional is
\begin{eqnarray}\label{ALM-KV}
    & \inf_{u,g} \int_{\Omega} R(|d_2|) + \frac{\alpha}{2} \int_{\Omega} |f-K(u+\Delta g)|^2 dx + \lambda \||d_1|\|_{L^1}\\
    & + \frac{r_1}{2} \|z-g-b_1\|^2 + \frac{r_2}{2} \|d_1 - \nabla z - b_2\|^2 + \frac{r_3}{2} \|d_2 - \nabla u - b_3\|^2.
\end{eqnarray}
with the Lagrange multipliers $b_1,b_2,b_3$ and $r_1,r_2,r_3 > 0$. 

The proposed iterative algorithm for the discretized problem \eqref{KV-Jung} is as follows:
\begin{equation}\label{ALM-iter}
\begin{split}
        & (u^{k+1},g^{k+1}) \in \mathrm{arg}\min_{u,g} \{ \frac{\alpha}{2} \|f-K(u+\Delta g)\|^2 \\
        & + \frac{r_1}{2} \|z^k-g-b_1^k\|^2 + \frac{r_3}{2} \|d_2^k - \nabla u - b_3^k\|^2\}, \\
        & z^{k+1} \in \mathrm{arg}\min_{z} \frac{r_1}{2} \|z-g^{k+1}-b_1^k\|^2 + \frac{r_2}{2} \|d_1^k - \nabla z - b_2^k\|^2, \\
        & d_1^{k+1} \in \mathrm{arg}\min_{d_1} \lambda \||d_1|\|_1 + \frac{r_2}{2} \|d_1 - \nabla z^{k+1} - b_2^k\|^2,\\
        & d_2^{k+1} \in \mathrm{arg}\min_{d_2} \|R(|d_2|)\|_1 + \frac{r_3}{2} \|d_2 - \nabla u^{k+1} - b_3^k\|^2,\\
        & b_1^{k+1} = b_1^k - (z^{k+1} - g^{k+1}),\\
        & b_2^{k+1} = b_2^k - (d_1^{k+1} - \nabla z^{k+1}),\\
        & b_3^{k+1} = b_3^k - (d_2^{k+1} - \nabla u^{k+1}).
\end{split}
\end{equation}
where $\||d|\|_1 = \sum_{i,j=1,\cdots,N} |d|_{i,j}$.

To solve the subproblem for $(u^{k+1},g^{k+1})$ in \eqref{ALM-iter}, the optimality condition reads 
\begin{eqnarray}
    & \alpha K^*(Ku - f + K\Delta g) + r_3 \mathrm{div}(d_2^k - \nabla u - b_3^k) = 0,\\
    & \alpha \Delta^* K^*(K\Delta g - f + Ku) - r_1 (z^k-g-b_1^k) = 0.
\end{eqnarray}
which can be efficiently solved via Fast Fourier Transform (FFT) implementation \cite{2007A,2010Augmented} as follows.

The author of \cite{doi:10.1137/140967416} proposed to obtain $u$ by fixing $g$,
\begin{equation}
    \mathcal{F}(u^{k+1}) = \frac{ \alpha \mathcal{F}(K^*) (\mathcal{F}(f)-\mathcal{F}(K)\mathcal{F}(\Delta)\mathcal{F}(g^k)) - r_3 \mathcal{F}(\mathrm{div}) \mathcal{F}(d_2^k - b_3^k) }{ \alpha \mathcal{F}(K^*)\mathcal{F}(K) - r_3 \mathcal{F}(\Delta) }
\end{equation}
and $g$ is obtained by fixing $u$,
 \begin{equation}
    \mathcal{F}(g^{k+1}) = \frac{\alpha \mathcal{F}(\Delta^*)\mathcal{F}(K^*) (\mathcal{F}(f)-\mathcal{F}(K)\mathcal{F}(u^{k+1})) + r_1\mathcal{F}(z^k-b_1^k)}{\alpha \mathcal{F}(\Delta^*)\mathcal{F}(K^*)\mathcal{F}(K)\mathcal{F}(\Delta) + r_1},
\end{equation}
where $\mathrm{div},\Delta,K$ can be viewed as convolution operators by considering the periodic boundary conditions, and $\mathcal{F}(\cdot)$ is the two-dimensional Fourier transform function.

The minimizing solution $z^{k+1}$ in \eqref{ALM-iter} satisfies
\begin{equation}
    (r_1 - r_2 \mathcal{F}(\Delta)) \mathcal{F}(z^{k+1}) = r_1\mathcal{F}(g^{k+1}+b_1^k) - r_2 \mathcal{F}(\mathrm{div}) \mathcal{F}(d_1^k - b_2^k).
\end{equation}

Solution $d_1^{k+1}$ of the problem \eqref{ALM-iter} have closed form solution using the shrinkage operator \eqref{shrink}:
\begin{equation}
    \mathrm{shrink}(\nabla z^{k+1} + b_2^k; 1/r_2)
\end{equation}


If $R(u) = |\cdot|$, solution $d_2^{k+1}$ of problem \eqref{ALM-iter} can be solved by:
\begin{equation}
    \mathrm{shrink}(\nabla u^{k+1} + b_3^k; 1/r_3).
\end{equation}
If $R(u) = \phi_a(\cdot),\quad a>0$ defined in \eqref{first}, it can be determined by Proposition 3.2 in \cite{2023A}.

Assume the first minimization of \eqref{ALM-iter} can be exactly solved, a convergence analysis of the proposed algorithm is discussed in \cite{doi:10.1137/140967416}.






==> KR_denoising/Article/Other/sinkhorn_TV.tex <==
\subsection{Variational Problems with entropic regularized OT}\label{sinkhorn}

%In \cite{2014Iterative, 2016Generalized}, %Wasserstein distances has been used as a data fidelity to perform computerized tomography and the image denoising model (\ref{Reg}) mentioned above.

The paper \cite{2015A} propose a computational framework to minimize the energy of problem (\ref{Reg}) for image denoising problem. While the algorithm for models (\ref{Reg}) and (\ref{KR-pro}) uses the usual Wasserstein (unregularized) distance, the paper \cite{2015A} propose to add entropic regularization to the OT distance, and the dual formulation of such Wasserstein variational problems can be implemented by simpler and faster numerical scheme.

Suppose the Kantorovitch formulation of Wasserstein distance (\ref{Kan}) is discretized on an uniform rectangular grid with $n=N \times N$ pixels $(z_i)_{i=1}^n$, 
then the metric is $M_{ij} = \|z_i-z_j\|^{\ell},(i,j)\in\{1,\cdots,n\}^2$.
Given two discrete probability distributions $p,q$ and the set of couplings $U(p,q) = \{X:X \mathbf{1}_n = p,X^T \mathbf{1}_n = q\}$, %and the entropic regularizaiton is $\gamma=\frac{1}{\sqrt{n}}$,
the entropy-regularized Wasserstein distances and its dual formulation are
\begin{align*}
     W_{\gamma}(p,q)& = \min_{X \in U(p,q)} \langle M, X\rangle + \gamma X\log X,\\
    & = \max_{(u,v)} \langle u,p\rangle + \langle v,q\rangle - \gamma \sum \exp(\frac{1}{\gamma}(u_i + v_j - M_{ij}) - 1), \gamma>0,
\end{align*}

Denote the the Wasserstein distance for a fixed probability $q$ as $H_q(p) = W_{\gamma}(p,q)$, 
then \cite{2015A} propose that the computation of the Fenchel-Legendre transform of $H_q(p)$, defined as $H_q^*(p) = \max_p \langle p,q\rangle - H_q(p)$,
and its derivatives has closed forms as
\begin{align}
    & H_q(p)^* = \gamma (E(q) + \langle q \log K\alpha\rangle), \\
    & \nabla H_q(p)^*  = \alpha \circ (K\frac{q}{K\alpha}), \alpha = e^{p/\gamma},K = e^{-M/\gamma}.
\end{align}

The image denoising model for a given image $q$ is 
\begin{eqnarray}
      \min_p w H_q(p) + \beta F(\mathcal{A}p), 
\end{eqnarray}
where the $F(\mathcal{A}p)$ is the total variation defined as $\mathcal{A} = \nabla, F(\cdot) = \|\cdot\|_2$. 
%is that the unregularized Wasserstein distance is used , while the entropic regularized transport is used here. 

%The Fenchel-Rockafelear dual problem is 
%\begin{eqnarray}
%    & \min_v w H_q^*(u) + F^*(v) + l_H(u,v), \\
%    & H = \{(u,v): \mathcal{A}^*v + w u  = 0\},
%\end{eqnarray}
%and the primal-dual relationships read $p = \nabla H_q(u)^*$.
%The simplest algorithm to solve $\min_x F(x) + G(x)$ is 
%This can be solved by the Forward-Backward algorithm, called sinkhorn-TV, whose iteration read
%\begin{eqnarray}
%    & v^{\ell+1} = \mathrm{Prox}_{\tau F^*} ( v^{\ell} + \tau \mathcal{A} \nabla H_q^*( - \mathcal{A}^* v^{\ell}/w) ),
   % & \mathrm{Prox}_{\tau F^*} (p)_i = \frac{p_i}{\min\{1, \lambda/\|p_i\|_{2}\}},i=1,2,\cdots,n,
%\end{eqnarray}

The matrix multiplication with Gibbs kernel $K = e^{-M/\gamma}$ is a filtering with a Gaussian kernel, which may leads to storage problem.
For Wasserstein-2 metric, i.e., $\ell = 2$, this can be solved efficiently by 'kernel seperate' \cite{2015Convolutional}, and for Wasserstein-1 metric, i.e., $\ell = 1$, the matrix multiplication can be solved a recently proposed Fast-sinkhorn method with lower computational cost\cite{2022Fast}.

%To circumvent , the "heat kernel" method is proposed in \cite{2015Convolutional} for solving OT on geometric domains. A method called Fast-Sinkhorn (FS) proposed recently to compute Wasserstein-1 distance on uniform grid can be used as an alternative.

==> KR_denoising/Experiment/Other_exp/KR_experiment.tex <==
\section{Numerical Experiment}
In this section, we present numerical experiments of the proposed denoising models for grayscale image (\ref{pro}) and color image(\ref{vomt-tv}) for image restoration and compare the experiment results with the traditional ROF model, i.e, the model with $L^2$-norm and TV regularizer.

Following \cite{2014Imaging}, for models with KR norm (\ref{KR}) and Vector OMT (\ref{vomt-tv}) as fidelty, we usually take $\lambda_1 = \infty$ so large that the respective constraint is inactive throughout. We can take $\lambda_2 = 1$ and then the regularizer strength $\beta = O(h^2)$ is tuned for better results, where $h$ is the mesh size usually taken as $h=0.1$.
%The regularizer strength $\beta=O(h^2)$ is tuned for better result.

In the Algorithm \ref{alg1}, we can take penalization parameters $r_z=O(h)$, $r_p=O(\beta)$.
For each outer iteration in ALM, we run the iterative algorithm (\ref{W1PD}) until the residual (\ref{residual}) is below $\epsilon$. 
Empirically, we have found that Algorithm \ref{alg1} converges even when $\epsilon=O(h^2)$ for the inner loops, so we usually set it as $h^2$.

The quality of the recovered images is measured by peak signal-to-noise ratio (PSNR), the measure of structural similarity (SSIM). And for measuring color image, we also use the S-CIELAB color metric as \cite{2019Color}.



\subsection{Grayscale Image Restoration}
In this section, we present several experiments for grayscale image denoising (the blur operator $K = I$) and deblurring to show that the proposed model (\ref{kr_new_rel}) help preserve image contrasts, compared with ROF model. 
%The smaller $\epsilon$ is, the more iteration it takes, the more accurate the sub-problem (\ref{zpro}) is solved.

%The metric of image quality is the peak signal-to-noise ratio (PSNR), signal to noise ratio (SNR), and the measure of structural similarity (SSIM).

\subsubsection{Cartoon-Texture decomposition}
    For cartoon-texture decomposition, according to \cite{2012Regularized, 2014Imaging}, KR-TV has favorable property.
    According to \cite{2006Structure}, the $L^1$-TV approach performs well when the texture part is known to be very structured, and G-TV is an improvement of TV-$L^2$.
    
    For the KR-TV decomposition, $\beta$ is chosen such that most texture is in the texture component, and then, the parameters of other models including $L^1$-TV and G-TV are adjusted such that the total variation of the cartoon part equals the total variation of cartoon parts of KR-TV.
    
    As shown in Figure \ref{car}, the texture component for KR-TV mainly contains texture, while some structure is mixed with texture for G-TV. 
    The results of the method in section (\ref{sinkhorn}) for Cartoon-Texture decomposition is similar to KR-TV.
    
    %But more texture part in the scarf and pants is removed in the image using KR-TV and Sinkhorn-TV than ROF.
%    \begin{figure}
%        \centering
%        \caption{Cartoon-Texture decomposition, psnr = 24.5 for ALM-KR with $\beta = 0.1h$, and psnr = 25.3 for ROF}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/ALM_KR/cartoon_kr_l2.jpg}
%    \end{figure}

%    \begin{figure}
%        \centering
%        \caption{Cartoon-Texture decomposition of ALM-KR, $\beta = 0.1h$}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/ALM_KR/cartoon_bar_l2_kr.jpg}
%    \end{figure}

%    \begin{figure}
%        \centering
%        \caption{Cartoon-Texture decomposition with Sinkhorn-TV(\ref{sinkhorn}) and L2-TV. The results of Cartoon-Texture decomposition using Sinkhorn-TV(\ref{sinkhorn}) is similar to ALM-KR.}
%        \includegraphics[width=\linewidth]{KR_denoising/figure/sinkhorn/cartoon_bar.jpg}
%    \end{figure}

%    \begin{figure}
%        \centering
%        \caption{Cartoon-Texture decomposition with ALM-KR, %Sinkhorn-TV(\ref{sinkhorn}) and ROF. The $L^2$-norm is $\|u-f\|_2=30$ for all three decomposition methods.}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/cartoon_comp.jpg}
%    \end{figure}
  \begin{figure}
    \centering
    \subfigure[$L^1$-TV]{
        \begin{minipage}{0.2\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/cartoon_bar/l1_5.2e3.jpg}
    \end{minipage}
    }
    \subfigure[G-TV]{
        \begin{minipage}{0.2\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/cartoon_bar/Gnorm_5.3e3.jpg}
    \end{minipage}
    }
    \subfigure[KR-TV]{
        \begin{minipage}{0.2\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/cartoon_bar/kr_5.12e3.jpg}
    \end{minipage}
    }
    \subfigure[method in (\ref{sinkhorn})]{
        \begin{minipage}{0.2\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/cartoon_bar/FS_tv_w_0.1_5.14e3.jpg}
    \end{minipage}
    }
    %\subfigure[FS-TV]{
    %    \begin{minipage}{0.2\linewidth}
        %\caption{FS-TV}
    %    \centering
     %   \includegraphics[width=\linewidth]{KR_denoising/figure/ALM_KR/cartoon/fs_tv_bar_car_63200.jpg}
    %\end{minipage}
    %}
    
    \subfigure[]{
    \begin{minipage}{0.2\linewidth}
        %\caption{$u-f+100$}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/cartoon_bar/l1_5.2e3_res.jpg}
    \end{minipage}
    }
    \subfigure[]{
        \begin{minipage}{0.2\linewidth}
        \centering
        %\caption{$u-f+100$}
        \includegraphics[width=\linewidth]{KR_denoising/figure/cartoon_bar/Gnorm_5.3e3_res.jpg}
    \end{minipage}
    }
    \subfigure[]{
        \begin{minipage}{0.2\linewidth}
        \centering
        %\caption{$u-f+100$}
        \includegraphics[width=\linewidth]{KR_denoising/figure/cartoon_bar/kr_5.12e3_res.jpg}
    \end{minipage}
    }
    \subfigure[]{
        \begin{minipage}{0.2\linewidth}
        \centering
        %\caption{$u-f+100$}
        \includegraphics[width=\linewidth]{KR_denoising/figure/cartoon_bar/FS_tv_w_0.1_5.14e3_res.jpg}
    \end{minipage}
    }
    %\subfigure[$u-f+100$]{
    %    \begin{minipage}{0.2\linewidth}
        %\caption{$u-f+100$}
    %    \centering
    %    \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/cartoon/fs_tv_bar_car_63200rof_res.jpg}
    %\end{minipage}
    %}
    \caption{Cartoon-Texture decomposition with $L^1$-TV, G-TV, KR-TV and the method in (\ref{sinkhorn}). }
    \label{car}
\end{figure}


\subsubsection{Results Comparison of Different Models}

In Fig.\ref{Fig:but},  The residual images illustrate that the KR-TV model sweeps fewer meaningful signals as noise than ROF model and thus helps retain image contrast.

    \begin{table}[htb]   
        \begin{center}   
        \caption{Comparison of PSNR(SSIM) results of restored butterfly image with Gaussian noise $\sigma=25/255$ using different algorithm with mesh size $h=1$, and the regularizer strength $\beta$. } 
        \label{table:1} 
        \begin{tabular}{|c|c|c|c|}   
        \hline   \textbf{PSNR}      & \textbf{PD-KR(\ref{PD-KR})}    & \textbf{ALM-KR(\ref{ALM-KR})}    & \textbf{Method(\ref{sinkhorn})} \\% &  \textbf{FS-TV}\\   
        \hline   $\beta = 0.6h^2$   & 27.47(0.847)      & 27.66(0.825)       &  26.55(0.738)               \\% & 27.51(0.840)\\  
        \hline   $\beta = 1h^2$     & 27.48(0.848)      & 27.48(0.847)      
         & 27.57(0.811)          \\% & 26.60(0.833)\\ 
        \hline   $\beta = 1.5h^2$   & 26.82(0.841)      & 26.71(0.840)         & 27.6(0.834)           \\% & 24.7(0.760)\\      
        \hline   
        \end{tabular}   
        \end{center}   
    \end{table}

%    \begin{figure}
%        \centering
%        \caption{Comparision of GD-KR and ROF, $h=1/N$}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/GD-KR/25gau_but.jpg}
%    \end{figure}

%    \begin{figure}
%        \centering
%        \caption{Comparision of the denoised images using ALM-KR and ROF. A Gaussian noise $\mathcal{N}(0,\sigma),\sigma = 25/255$ is added to the image.}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/ALM_KR/25gau_but.jpg}
%    \end{figure}

\begin{figure}
    \centering
    \subfigure[Noise-free image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= 0.9\linewidth]{KR_denoising/figure/ALM_KR/eps/05.png}
        %\caption{ROF 27.83(0.845)}
    \end{minipage}
    }
    \subfigure[Degraded image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= 0.9\linewidth]{KR_denoising/figure/ALM_KR/eps/but_25gau.eps}
        %\caption{$u-f+100$}
    \end{minipage}
    }
    
    \subfigure[ROF]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= 0.9\linewidth]{KR_denoising/figure/new_model/monarch/rof_27.29_0.850.jpg}
        %\caption{ROF 27.83(0.845)}
    \end{minipage}
    }
    \subfigure[]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= 0.9\linewidth]{KR_denoising/figure/new_model/monarch/rof_27.29_0.850_res.jpg}
        %\caption{$u-f+100$}
    \end{minipage}
    }
    
    \subfigure[G-TV]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= 0.9\linewidth]{KR_denoising/figure/new_model/monarch/g_l2_tv_mu0.06_lam0.3_27.81_0.860.jpg}
        %\caption{KR-TV 27.96(0.853)}
    \end{minipage}
    }     
    \subfigure[]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/new_model/monarch/g_l2_tv_mu0.06_lam0.3_27.81_0.860_res.jpg}
        %\caption{$u-f+100$}
    \end{minipage}
    }

    \subfigure[KR-TV]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= 0.9\linewidth]{KR_denoising/figure/new_model/monarch/kr_l2_tv_lam2_1_lam0.3_27.3_0.850.jpg}
        %\caption{KR-TV 27.96(0.853)}
    \end{minipage}
    }     
    \subfigure[]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/new_model/monarch/kr_l2_tv_lam2_1_lam0.3_27.3_0.850_res.jpg}
        %\caption{$u-f+100$}
    \end{minipage}
    }
    \caption{Grayscale image denoising results of ROF, G-TV and KR-TV for image denoising on "butterfly" image with Gaussian noise $\mathcal{N}(0,\sigma),\sigma = 25/255$.}
    \label{Fig:but}
\end{figure}

%    \begin{figure}
%        \centering
%        \caption{Comparision of the denoised images using Sinkhorn-TV and $L^2$-TV. For Sinkhorn-TV the entropic regularization is $\gamma=1/4$, $\beta=h$. }
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/sinkhorn/25gau_but.jpg}
%    \end{figure}


%    \item Performance impact of different Gaussian noise level.
%    More meaningful signals are swept as noise by the ROF model than the KR-TV model in the residual images with different noise level .
%    Although the PSNR of KR-TV model may not be optimal, it is comparable to that of ROF model, and the SSIM of KR-TV model is usually higher especially for high level noise.
%    \begin{figure}
%        \centering
%        \caption{Gaussian noise $\sigma=40/255$}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/ALM_KR/40gau_star.jpg}
%    \end{figure}

%    \begin{figure}
%        \centering
%        \caption{Gaussian noise $\sigma=50/255$}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/ALM_KR/50gau_pep.jpg}
%    \end{figure}

%    \begin{figure}
%        \centering
%        \caption{Gaussian noise $\sigma=75/255$}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/ALM_KR/75gau_pep.jpg}
%    \end{figure}

%    \item Generalizability to other noise type
    
%    \begin{figure}
%        \centering
%        \caption{Poisson noise $\lambda=0.4$}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/ALM_KR/0.4poi_star.jpg}
%    \end{figure}

%    \begin{figure}[htbp]
%    \centering
%    \includegraphics[width=\textwidth]{KR_denoising/figure/tgv_kr_bsd_4.eps} % 替换example.eps为您的图片文件名
%    \caption{TGV}
%    \label{fig:epsimage}
%    \end{figure}


%\input{KR_denoising/KR_regularizer}

\subsubsection{Convergence Results of the proposed model (\ref{pro})}


To monitor the convergence of the iterative process of sub-problem (\ref{zpro}), we check the following values,
    the residual of PDHG $R^k$ (\ref{residual}), and the constraint \begin{equation}\label{con}
        \frac{\|z-f+ \mathrm{div}_h m_h\|_F}{\|z-f\|_F}.
    \end{equation}
    
\begin{figure}
    \centering
    \subfigure{
        \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/conv/pdhg_res_1.jpg}
    \end{minipage}
    }
    \subfigure{
        \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/conv/pdhg_con_1.jpg}
    \end{minipage}
    }

    \caption{The plots of the residual of PDHG $R^k$ and the constraint (\ref{con}) versus iteration of the sub-problem (\ref{zpro}) in one iteration of ALM for the experiment in Fig.\ref{Fig:but} using the proposed model.}
\end{figure}



==> KR_denoising/Experiment/Other_exp/KR_regularizer.tex <==
\subsubsection{Performance impact of different regularization term}
\begin{enumerate}
        \item The first order regularizer from \cite{2023A} for models with $L^2$ and KR norm for image denoising and deblurring. 
        
    $R(u)$ can be taken as different regularizers including the total generalized variation (TGV) \cite{Bredies2010TotalGV} and the first order regularization term $R(u) = \phi_a(\nabla u),\;a>0$ in \cite{2023A}.
    $\phi_a$ is defined as 
    \begin{equation}\label{first}
    \begin{split}
    \phi_a(x) = \left \{
        \begin{array}{lr}
            \frac{1}{2a} x^2,                 & |x|\leq a,\\
            a \ln |x| + \frac{a}{2} - a\ln a, & |x|> a,
        \end{array}
        \right.	
    \end{split}
    \end{equation}
        
    The residual images illustrate that the model with the first order regularizer sweeps fewer meaningful signals as noise than that with TV regularizer and thus helps retain image contrast .

    
    %\begin{figure}
    %    \centering
    %    \caption{$L^2$ norm and KR norm with zhu regularization($a = 0.5$)}
   %     \includegraphics[width=0.9\linewidth]{KR_denoising/figure/ALM_KR/zhu/gau_kr_l2_zhu_but.jpg}
    %\end{figure}

%    \begin{figure}
%        \centering
%        \caption{$L^2$ norm and KR norm with zhu regularization($a = 0.5$), $\beta=1.5h$ for ALM-KR}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/ALM_KR/zhu/25gau_zhu.jpg}
%    \end{figure}


    \item KR norm model with the total generalized variation (\ref{tgv}) perserve the texture better, while KR-TV remove all the texture.
\begin{figure}
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= 0.7\linewidth]{KR_denoising/figure/ALM_KR/bsd004/rof_0.1_28.84_0.767.jpg}
        \caption{ROF 28.84(0.767)}
    \end{minipage}
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= 0.7\linewidth]{KR_denoising/figure/ALM_KR/bsd004/rof_0.1_28.84_0.767_res.jpg}
        \caption{$u-f+100$}
    \end{minipage}

    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= 0.7\linewidth]{KR_denoising/figure/ALM_KR/bsd004/kr_0.1_28.46_0.766.jpg}
        \caption{KR-TV 28.46(0.766)}
    \end{minipage}
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{KR_denoising/figure/ALM_KR/bsd004/kr_0.1_28.46_0.766_res.jpg}
        \caption{$u-f+100$}
    \end{minipage}  
    
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= 0.7\linewidth]{KR_denoising/figure/ALM_KR/bsd004/tgv_0.1_28.47_0.775.jpg}
        \caption{$L^2$-TGV 28.47(0.775)}
    \end{minipage}
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{KR_denoising/figure/ALM_KR/bsd004/tgv_0.1_28.47_0.775_res.jpg}
        \caption{$u-f+100$}
    \end{minipage}  
    
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= 0.7\linewidth]{KR_denoising/figure/ALM_KR/bsd004/kr_tgv_0.1_28.5_0.752.jpg}
        \caption{KR-TGV 28.5(0.752)}
    \end{minipage}
    \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{KR_denoising/figure/ALM_KR/bsd004/kr_tgv_0.1_28.5_0.752_res.jpg}
        \caption{$u-f+100$}
    \end{minipage}  
    \caption{restored images with gaussian noise $\sigma=25/255$ using models with KR norm and $L^2$ norm as fidelity and TV and TGV as regularizer .}
\end{figure}

\end{enumerate}

==> KR_denoising/Experiment/Other_exp/convergence.tex <==
\subsubsection{Convergence}
    To monitor the convergence of Algorithm \ref{alg1}, we check the following relative residual as in \cite{2023A}, 
    \begin{equation}\label{res-pz}
        R_p^k = \frac{\|p^k-\nabla u^k\|_F}{|\Omega|},\; R_z^k = \frac{\|z^k-K*u^k\|_F}{|\Omega|},
    \end{equation}
    and the relative error of the solution $u^k$
    \begin{equation}\label{rel-u}
        \frac{\|u^k-u^{k-1}\|_F}{\|u^{k-1}\|_F}
    \end{equation}
    where $|\Omega|$ is the area of $\Omega$, and the values are plotted in log-scale in the figure.
    
\begin{figure}
    \subfigure{
        \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/conv/z_rel_lis_1.jpg}
    \end{minipage}
    }
    \subfigure{
        \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/conv/p_rel_lis_1.jpg}
    \end{minipage}
    }
    \subfigure{
        \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/conv/u_rel_lis_1.jpg}
    \end{minipage}
    }     
    \subfigure{
        \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/ALM_KR/conv/energy.jpg}
        %\caption{$u-f+100$}
    \end{minipage}
    }
    \caption{The plots of the relative residual $R_z^k$ and $R_p^k$ (\ref{res-pz}), the relative error of $u^k$ (\ref{rel-u}) and the energy (\ref{KR-pro}) versus iteration
    for the experiment in Fig.\ref{Fig:but} using the proposed model. All the quantities are presented in \textit{log-scale}}
\end{figure}



    To monitor the convergence of the iterative process of subproblem (\ref{zpro}), we check the following values and plot them in one outer iteration for illustration,
    the relative residual of PDHG (\ref{residual}), and the constraint $\frac{\|z-f+ \mathrm{div}_h m_h\|_F}{\|z-f\|_F}$,
    %the value of the KR norm function (\ref{W1PD}), the value of primal function $\lambda_2\|m_h\|_2$.
%    \begin{figure}
%        \centering
%        \caption{convergence of subproblem (\ref{zpro})}
%        \includegraphics[width=0.9\linewidth]{KR_denoising/figure/ALM_KR/sub_pro_convergence.jpg}
%    \end{figure}


To monitor the convergence of ALM Algorithm for VOMT-TV in section \ref{alm-vomt}, we check the following values.

\begin{figure}
    \subfigure{
        \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/RGB/p_err_epi_h2_10beta_rp_5h_rz.jpg}
    \end{minipage}
    }
    \subfigure{
        \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/RGB/z_err_epi_h2_10beta_rp_5h_rz.jpg}
    \end{minipage}
    }
    \subfigure{
        \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/RGB/u_err_epi_h2_10beta_rp_5h_rz.jpg}
    \end{minipage}
    }     
    \subfigure{
        \begin{minipage}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/RGB/energy_epi_h2_10beta_rp_5h_rz.jpg}
        %\caption{$u-f+100$}
    \end{minipage}
    }
    \caption{The plots of the relative residual $R_p^k$ and $R_p^k$, the relative error of $u^k$ and the energy (\ref{vomt-tv}).}
\end{figure}


    To monitor the convergence of the iterative process of subproblem (\ref{zpro-vomt}), we check the following values and plot them in one outer iteration for illustration,
    the relative residual of PDHG (\ref{res-vomt}), the value of subproblem (\ref{zpro-vomt}), the value of primal function $\|\vec{m}\|_u$, and $\|\vec{w}\|_w$,

    \begin{figure}
        \centering
        \caption{convergence of subproblem (\ref{zpro-vomt}) in one outer iteration with $\alpha=0.1$.}
        \includegraphics[width=\linewidth]{KR_denoising/figure/RGB/sub_conv_vomt.jpg}
    \end{figure}


Another formulation of KR norm (\ref{KR-norm}), called the cascading or dual formulation, is given in \cite{2014Imaging}, and we quote it here.
\begin{theorem}
    (Cascading formulation) Let $\Omega$ be open, convex, and bounded, and let $\lambda = (\lambda_1,\lambda_2) \geq 0$, $\mu\ in L^1(\Omega)$. The dual formulation of (\ref{KR-norm}) is 
\begin{equation}\label{KR-dual}
    \begin{split}
        \|\mu\|_{KR,\lambda} & = \min_{\vec{v} \in L^1(\Omega,\mathbb{R}^2)}  \lambda_1 \|\mu + \mathrm{div} \vec{v}\|_{L^1} + \lambda_2\|\vec{v}\|_{L^1}\\
        & = \min_{\vec{v} \in L^1(\Omega,\mathbb{R}^2)} \max_{\phi \in L^1(\Omega,\mathbb{R})} \int_\Omega \phi(\mu + \mathrm{div} \vec{v})dx - I_{|\cdot|_{\infty}\leq \lambda_1}(\phi) + \lambda_2\|\vec{v}\|_{L^1}
    \end{split}
\end{equation}
where $\|\vec{v}\|_{L^1} = \sup_{|\vec{f}|\leq 1} \int_\Omega \vec{f} d \vec{v}$.
%$\mathrm{div} \vec{v}$ is taken in $\bar{\Omega}$ or any open set $U$ containing $\bar{\Omega}$.
\end{theorem}



\begin{figure}
    \centering
    \subfigure{
        \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/conv/z_rel_lis_1.jpg}
    \end{minipage}
    }
    \subfigure{
        \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/conv/p_rel_lis_1.jpg}
    \end{minipage}
    }
    
    \subfigure{
        \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/conv/u_rel_lis_1.jpg}
    \end{minipage}
    }     
    \subfigure{
        \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/ALM_KR/conv/energy.jpg}
        %\caption{$u-f+100$}
    \end{minipage}
    }
    \caption{The plots of the residual of PDHG $R^k$ and the constraint (\ref{con}) versus iteration of the sub-problem (\ref{zpro}) in one iteration of ALM. 
    The plots of $R_z^k$ and $R_p^k$ (\ref{res-pz}), the relative error of $u^k$ (\ref{rel-u}) and the energy (\ref{KR-pro}) versus iteration for the experiment in Fig.\ref{Fig:but} using the proposed model.}
\end{figure}

==> KR_denoising/Experiment/Other_exp/sisr.tex <==
\subsubsection{Image deblurring and Single Image Super-Resolution (SISR)}



    %\begin{figure}
    %    \centering
    %    \caption{The scale factor $K=4$, $H$ is Gaussian of std 1, hsize=9, $\sigma=7.65/255$}
    %    \includegraphics[width=\linewidth]{KR_denoising/figure/RGB/super_rgb_K4_rho0.01.jpg}
    %\end{figure}
%    \begin{figure}
%        \centering
%        \caption{Performance impact of zhu regularizer ($a=0.2$) for L2 and KR norm, $h=25,\sigma=1.6$ for blurring,$\sigma=15/255$ Gaussian noise.}
%        \includegraphics[width=\linewidth]{KR_denoising/figure/RGB/zhu_1.6blur_15gau_cos.jpg}
%    \end{figure}

\begin{figure}
    \centering
    \subfigure[]{    
    \begin{minipage}{0.22\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/RGB/starfish/star_1.6_25_5.eps}
        %\caption{KR-TV (21.64dB)}
    \end{minipage}}
    \subfigure[]{
        \begin{minipage}{0.22\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/RGB/starfish/rof_1.6_25_5_27.00_0.959.eps}
        %\caption{NCSR (22.67dB)}
    \end{minipage}
    }
    \subfigure[ ]{
        \begin{minipage}{0.22\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/RGB/starfish/vomt_1.6_25_5_27.15_0.963.eps}
        %\caption{LR image}
    \end{minipage}
    }
    \subfigure[]{
        \begin{minipage}{0.22\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/RGB/starfish/ncsr_1.6_25_5_27.57_0.952.eps}
        %\caption{ROF (21.52dB)}
    \end{minipage}
    }
    \caption{The blurred and noise image is obtained by applying a $25 \times 25$ Gaussian kernel with standard deviation $\sigma=1.5$ and adding Gaussian noise $\sigma=5/255$. (a) Degraded image 24.1(0.926). (b) ROF 27.00(0.959). (c) VOMT-TV 27.15(0.963). (d)NCSR 27.57(0.952).}
\end{figure}



\begin{figure}
    \centering
    \subfigure[]{
        \begin{minipage}{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/RGB/eps/K_4_9_1_5.eps}
        %\caption{LR image}
    \end{minipage}
    }
    \subfigure[]{
        \begin{minipage}{0.22\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/RGB/eps/rof_K_4_9_1_5.eps}
        %\caption{ROF (21.52dB)}
    \end{minipage}
    }
    \subfigure[]{    
    \begin{minipage}{0.22\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/RGB/eps/KR_K_4_9_1_5.eps}
        %\caption{KR-TV (21.64dB)}
    \end{minipage}}
    \subfigure[]{
        \begin{minipage}{0.22\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/RGB/eps/nscr_K_4_9_1_5.eps}
        %\caption{NCSR (22.67dB)}
    \end{minipage}
    }
    \caption{The image is blurred by a $9 \times 9$ Gaussian kernel with standard deviation $\sigma=1$, then downsampled by a scaling factor $\times 4$, The Gaussian noise $\sigma=5/255$ is added to the LR image. (a)Low resolution image. (b) ROF (21.52dB). (c) VOMT-TV (21.64dB). (d)NCSR  (22.67dB)}
\end{figure}

==> KR_denoising/Experiment/grayscale/1d.tex <==
In the following, we consider the model \eqref{Reg} with the Kantorovich optimal transport problem.
Let $\Omega=\{x_1,\cdots,x_n\}$ be the discretized space domain, then \eqref{Reg} can be reformulated as a linear problem (LP) \cite{2012Regularized}: 
\begin{equation}\label{W-LP}
    \begin{split}
        & \min_{\gamma,u} \sum_{i=1}^n \sum_{j=1}^n \frac{\lambda}{2} |x_i-x_j| \gamma_{ij} + \sum_{i=1}^n R(\nabla u_i), \\
         s.t.& \sum_{i=1}^n \gamma_{ij} = f_j, j =1,\cdots,n,\\
        & \sum_{j=1}^n \gamma_{ij} = u_i, u_i\geq 0, i =1,\cdots,n,\\
        %& \sum_{i=1}^n u_i = \sum_{j=1}^n f_j = 1,
    \end{split}
\end{equation}
with given initial data $f_j$. The transport map matrix $\gamma$ and distribution $u$ are unknown. When $R$ is convex, the linear problem \eqref{W-LP} can be directly solved by convex optimization solvers using an interior-point-method. 

In Figure \ref{Fig:1d}, we present numerical results for the linear problem \eqref{W-LP} in one dimension.
We consider different convex regularization functionals including $R(x)=|x|,R(x)=|x|^2$ and $R(x)=\log \cosh |x|$\cite{2007GarImage}. {\color{red} can we use log-TV for E(u)?} and optimize it with CVX solvers in MATLAB. 
%and compare the numerical results with our model \eqref{kr_new_rel}.
Our initial condition is a Gaussian curve with mean zero and variance one (colored in blue). %satisfying $h\sum_{j=1}^n f_j = 1, h=10/n$. $h$ is the mesh size and we take $\beta=h^2$.
{\color{red}The legends are missing...}


%For our model and \eqref{W-LP}, and the plateau becomes wider and flatter, but the total mass is still the same as $\sum_{j=1}^n f_j$ in the limit $\lambda \to 0$. 
%For a large parameter $\lambda$, the minimizer is the same as the initial plateau. 
{\color{red}1. for the plots in Fig. 1, we may consider fewer choices (say 3 different parameters) of $\lambda$ or $\alpha$; 2. can we specify the purpose of presenting this one-dimensional example?}

 %{\color{red}the minimization of \eqref{Kan}?} 
The method \eqref{W-LP} is only efficiently solvable in one dimension due to the fact that an $n = N \times N$ image yields an $N^2 \times N^2$ matrix $\gamma$.

%Therefore, for two dimensional real images, the Benamou-Brenier formulation \eqref{flu} is considered in \cite{2012Regularized}.
%The KR-TV model \eqref{KR-pro} is proposed in \cite{2014Imaging} and solved by the inertial forward-backward primal-dual method from \cite{2015Pock}. 

%The W-TV and KR-TV models are convex optimizations, and the number of variables is small for one dimension case so that convex optimization solvers can be applied.

\begin{figure}
    \centering
    \subfigure[$R(x)=|x|$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/1d/gau-W-TV.jpg}
    \end{minipage}
    }
    \subfigure[$R(x)=|x|^2$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/1d/gau-W-diri.jpg}
    \end{minipage}
    }
    \subfigure[$R(x)=\log \cosh |x|$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/1d/log_cosh.jpg}
    \end{minipage}
    }
    \caption{Numerical results for \eqref{W-LP}.}
    \label{Fig:1d}
\end{figure}

\begin{comment}
    \subfigure[Log entropy]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/1d/log_ent.jpg}
    \end{minipage}
    }
        \caption{Numerical results for model \eqref{W-LP} different regularizaton for various $\lambda$ in one dimension case.}
    
        \subfigure[ROF]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/1d/ROF-1.jpg}
    \end{minipage}
    }
\end{comment}

==> KR_denoising/Experiment/grayscale/ADMM_KV.tex <==
\subsubsection{Comparison Between the KR-Log-TV Model \eqref{kr_new_rel_log} and the Vese and Osher's functional \eqref{VO}}

In Figure \ref{Fig:bar_rof}, we consider a noisy textured image corrupted with white Gaussian noise of standard deviation $\sigma=15$. 

We show denoising results using the ROF model with parameter $\alpha=20$. 
Then we show results obtained with the KR-TV model \eqref{kr_new_rel} with $\lambda=4$, for the same parameter $\alpha=20$, which should constrast with the Vese and Osher's functional \eqref{VO} in the case $p=1$ in \cite{vese2003modeling}. 
However, for decreasing $\lambda$, more texture appears in the $v$ component by the proposed model, but also more noise is kept.
The model \eqref{uvw} from \cite{aujol2005dual} provides a solution for separating noise from texture.
\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_1/bar_1.eps}
    \end{minipage}
    }
    \subfigure[Noisy Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_1/bar_1_15.eps}
    \end{minipage}
    }
    \subfigure[ROF $u$ 24.2]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_1/rof_alp20_u_24.22.eps}
    \end{minipage}
    }
    \subfigure[$f-u+100/25$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_1/rof_alp20_f-u_18.eps}
    \end{minipage}
    }

    \subfigure[KR-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_1/kr_alp20_lam4_u.eps}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_1/kr_alp20_lam4_v.eps}
    \end{minipage}
    }
    \subfigure[$u+v$ 24.47]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_1/kr_alp20_lam4_u+v_24.47.eps}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_1/kr_alp20_lam4_f-u-v.eps}
    \end{minipage}
    }
    
    \caption{The first result is obtained by the ROF model with $\alpha=20$. 
    The second result is obtained by using the KR-TV model \eqref{kr_new_rel} with $\alpha=20$ and $\lambda=4$.
    }
    \label{Fig:bar_rof}
\end{figure}


%Let $m = (m_1,m_2) = \nabla g$, i.e., $v = \mathrm{div}(\nabla g ) = \Delta g$ as in \cite{garnett2011modeling}, the proposed model \eqref{kr_new_rel_log} is written as, 
%\begin{equation}\label{KV-lip}
%    \inf_{u,g} R(\nabla u)+ \frac{\alpha}{2} \int_{\Omega} |f-K * u-\Delta g|^2 dx + \lambda \||\nabla g|\|_{L^1},
%\end{equation}
%which should contrast with the OSV model \eqref{osv} %and model \eqref{KV-Jung}. 
%The solution of the model \eqref{KV-lip} can be obtained by the ADMM algorithm for the model \eqref{KV-Jung}.

In Figure \ref{Fig:bar_1_KV_log_15}, we show the results using the model \eqref{KV-Jung} with $E(u)=\mathrm{TV}(u)$, which should contrast with the proposed model \eqref{kr_new_rel} by letting $m = (m_1,m_2) = \nabla g$, i.e., $v = \mathrm{div}(\nabla g ) = \Delta g$ as in \cite{garnett2011modeling}.
The model \eqref{KV-Jung} separately regularizes the cartoon components $u$ and texture components $v=\Delta g$ with different norms.

%The comparison shows that the model \eqref{KV-Jung} denoises the texture part while successfully preserving textures, while the ROF model tends to smooth out texture in some region.

\begin{figure}
    \centering
%    \subfigure[Model \eqref{KV-lip} $u$ 25.37]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/ADMM_log_tv/kr_lam1e2_bet0.7_zhu_a5_u_25.4.jpg}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/25$]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/ADMM_log_tv/kr_lam1e2_bet0.7_zhu_a5_f-u_14.7.jpg}
%    \end{minipage}
%    }
    
    \subfigure[Model \eqref{KV-Jung} $u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/ADMM_log_tv/kr_lam20_bet3_u.jpg}
    \end{minipage}
    }
    \subfigure[$\Delta g + 100/25$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/ADMM_log_tv/kr_lam20_bet3_del_g.jpg}
    \end{minipage}
    }
    \subfigure[$u+\Delta g$ 25.13]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/ADMM_log_tv/kr_lam20_bet3_u+del_g_25.13.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-\Delta g +100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/ADMM_log_tv/kr_lam20_bet3_f-u-del_g_n_15.6.jpg}
    \end{minipage}
    }
    \caption{
        %The first result is obtained by model \eqref{KV-lip} with Log-TV with $\alpha=200,\lambda=0.7$.
        The result is obtained by model \eqref{KV-Jung} with TV with $\alpha=20,\lambda=3$. }
    \label{Fig:bar_1_KV_log_15}
\end{figure}



In Figure \ref{Fig:bar_1_kr_log_15}, we show results using the proposed KR-Log-TV model \eqref{kr_new_rel_log}. From the image $f-u+100/25$, we see that the KR-Log-TV preserve the contrast better.
\begin{figure}
    \centering
    \subfigure[KR-Log-TV $u$ 25.33]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_1/kr_zhu_a8_alp100_lam0.6_u_25.15.eps}
    \end{minipage}
    }
    \subfigure[$f-u+100/25$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_1/kr_zhu_a8_alp100_lam0.6_f-u_15.1.eps}
    \end{minipage}
    }
    
%    \subfigure[$L^2$-Log-TV $u$ 25.17]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/ADMM_log_tv/zhu_lam_10_a_5_u_25.17.jpg}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/25$]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/ADMM_log_tv/zhu_lam_10_a_5_f-u_n_14.9.jpg}
%    \end{minipage}
%    }
    \caption{%The first result is obtained by the $G$-TV model \eqref{g-pro-l2} with $\alpha=200,\mu=0.3$.
    The result is obtained by the KR-Log-TV model \eqref{kr_new_rel_log} with $\alpha=200,\lambda=0.7$.
    The removed noise part has the norm $\|f-u\|_F \approx 15$.}
    \label{Fig:bar_1_kr_log_15}
\end{figure}







==> KR_denoising/Experiment/grayscale/DCT.tex <==
\subsection{Cartoon-texture denoising algorithm}
The paper \cite{2003StaImage} proposed a novel method for separating images into texture and piecewise smooth parts.
    \begin{equation}\label{dct}
        \inf_{u,v} \mu_1 \|\mathcal{C} u \|_1 + \mu_2 \|\mathcal{D} v \|_1 + \frac{1}{2}\|f-u-v\|^2,
    \end{equation} 
where $\mathcal{D}$ denotes the overlapped local discrete cosine transforms (LDCTs) adapted to texture, and $\mathcal{C}$ is a transform adapted to the geometrical part of the image (for instance the curvelet transform). The noise $w=f-u-v$ is penalized through its $L^2$ norm.

The (Local) Discrete Cosine Transform (DCT): overlapping DCT transform with block size 32 for an overlap of 0.5.
\begin{equation}
    \inf_v \beta \|\mathcal{D} v \|_1 + \frac{\alpha}{2}\|f-u-v\|^2,
\end{equation}
is solved by soft thresholding the coefficient $\alpha=\mathcal{D}(f-u)$ with the $\delta$ threshold.

The paper \cite{cai2010} employed the unconstrained split Bregman algorithm to solve \eqref{dct}.

In \cite{}, the image restoration problem use two wavelet frame systems that can sparsely represent cartoons and
textures separately.
\begin{equation}
    \inf_{u,v} \mu_1 \|\lambda_1 \cdot W_1 u \|_{1,p_1} + \|\lambda_2 \cdot W_2 v \|_{1,p_2} + \frac{1}{2}\|f - K*(u+v)\|^2,    
\end{equation}
where $p_1,p_2$ are either 1 or 2.
The authors use Haar framelet for $W_1$ and expect $u$ to contain only the cartoon component of the image, and piecewise linear framelets for $W_2$ in order to properly model texture components.

\begin{figure}
    \centering
    \subfigure[Model \eqref{dct} $u$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/uvw_dct/uv_tv_alp10_dct_32_s_2_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/uvw_dct/uv_tv_alp10_dct_32_s_2_v.jpg}
    \end{minipage}
    }
    
    \subfigure[$u+v$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/uvw_dct/uv_tv_alp10_dct_32_s_2_u+v_27.45.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/uvw_dct/uv_tv_alp10_dct_32_s_2_f-u-v_n_48.jpg}
    \end{minipage}
    }
    \caption{Results using the model \eqref{dct} where $\|\mathcal{C} u \|_1$ is replaced by $\mathrm{TV}(u)$ for $\alpha=10,\delta=2\sigma$.}
\end{figure}



\begin{figure}
    \centering
    \subfigure[Model \eqref{dct} $u_1$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cur_dct/bar_mu1_h_3sig_mu2_s_2_u1.jpg}
    \end{minipage}
    }
    \subfigure[$u_2+100/25$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cur_dct/bar_mu1_h_3sig_mu2_s_2_u2.jpg}
    \end{minipage}
    }
    
    \subfigure[$u_1+u_2$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cur_dct/bar_mu1_h_3sig_mu2_s_2_u1+u2_27.45.jpg}
    \end{minipage}
    }
    \subfigure[$f-u_1-u_2+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cur_dct/bar_mu1_h_3sig_mu2_s_2_f-u1-u2_n_50.jpg}
    \end{minipage}
    }
    \caption{Results using the model \eqref{dct} for $\mu_1=3\sigma,\mu_2=2$.}
    \label{Fig:bar_cur_dct}
\end{figure}




==> KR_denoising/Experiment/grayscale/KR-TV.tex <==
We show the result $u$ and the residual using the proposed KR-TV model, compared with the results obtained with the ROF \eqref{rof}, the OSV \eqref{osv} and the $G$-TV model \eqref{g-pro-l2}.

The parameters $\alpha$ and $\lambda$ correspond to the ones in \eqref{kr_new_rel}. 
The larger $\alpha$ is, the smaller $|f-u-v|^2_{L^2}$ is, and we set $\alpha$ to be large.
For the proposed model, the smaller $\lambda$ is, the more $v$ contains information, and $\lambda$ is tuned such that the removed noise part has the norm $\|f-u\|_F = N\sqrt{\sum_{1\leq i,j\leq N} f_{ij}^2/N^2} \approx N\sigma$.

The parameter $\alpha$ for the ROF model \eqref{rof}, $\mu$ for the $G$-TV model and $\lambda$ for the OSV model are tuned to satisfy the constraint $\|f-u\|_F = N\sigma$.



In Figure \ref{Fig:u_n_pep}, the noisy image is corrupted by Gaussian noise with level $\sigma=15/255$, and the additive noise $n$ has the Frobenius norm $\|n\|_F = 15.0$.
\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/peppers/pep.jpg}
    \end{minipage}
    }
    \subfigure[Noisy Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/peppers/pep_15.jpg}
    \end{minipage}
    }
    
    \subfigure[ROF]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/peppers/rof_u_29.93.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/peppers/rof_f-u_n_14.9.jpg}
    \end{minipage}
    }
    
    \subfigure[$G$-TV]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/peppers/g_alp50_mu0.03_u_30.7.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/peppers/g_alp50_mu0.03_f-u_14.6.jpg}
    \end{minipage}
    }
    
    \subfigure[KR-TV]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/peppers/kr_lam2_alp50_u_29.55.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/peppers/kr_lam2_alp50_f-u_n_14.5.jpg}
    \end{minipage}
    }
    
    \subfigure[OSV]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/OSV/pep_15_admm_kv_lam4e1_bet2.5e2_u_29.8.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/OSV/pep_15_admm_kv_lam4e1_bet2.5e2_f-u_14.9.jpg}
    \end{minipage}
    }   
    \caption{Results using the ROF model with $\alpha=15$ and the proposed model \eqref{kr_new_rel} with parameter $\alpha=50$ and $\lambda=2$. }
    \label{Fig:u_n_pep}
\end{figure}


In Figure \ref{Fig:u_n_but}, we show the result $u$ and the residual using the ROF model and the results obtained with the proposed model.
The noisy image is corrupted by Gaussian noise with level $\sigma=25/255$, and the additive noise $n$ has the Frobenius norm $\|n\|_F = 25.0$.
\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/eps/05.png}
    \end{minipage}
    }
    \subfigure[Noisy Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/eps/but_25gau.eps}
    \end{minipage}
    }
    
    \subfigure[ROF]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/but_25/rof_u_27.35.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/but_25/rof_alp_10_f-u_n_24.1.jpg}
    \end{minipage}
    }
    
    \subfigure[$G$-TV]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/but_25/g_tv_mu_0.07_alp80_u_27.9.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/but_25/g_tv_mu_0.07_alp80_f-u_n_24.5.jpg}
    \end{minipage}
    }
    
    \subfigure[KR-TV]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/but_25/kr_lam1_alp80_u_27.45.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/but_25/kr_lam1_alp80_f-u_n_24.5.jpg}
    \end{minipage}
    }
    
    \subfigure[OSV]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/OSV/but_25_admm_kv_lam4e1_bet1.5e2_u_27.57.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/OSV/but_25_admm_kv_lam4e1_bet1.5e2_f-u_n_24.8.jpg}
    \end{minipage}
    }
    
    \caption{Results using the ROF model \eqref{rof} with $\alpha=10$, and the proposed model \eqref{kr_new_rel} with parameter $\alpha=80$ and $\lambda=1$ in and  in \eqref{rof}. }
    \label{Fig:u_n_but}
\end{figure}



\begin{figure}
    \centering
%    \flushright
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/01.png}
    \end{minipage}
    }
    \subfigure[Noisy Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/cam_20.jpg}
    \end{minipage}
    }
    
    \subfigure[ROF]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/rof_u_alp14_28.4.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/rof_u_f-u_n_19.9.jpg}
    \end{minipage}
    }    
    \subfigure[$L^2$-Log-TV]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/zhu_a5_alp4_u_28.4.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cam_20/zhu_a5_alp4_f-u_n_20.1.jpg}
    \end{minipage}
    }
    
    \subfigure[$G$-TV]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/g_mu0.06_alp200_u_28.37.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cam_20/g_mu0.06_alp200_f-u_n_20.4.jpg}
    \end{minipage}
    }
    \subfigure[$G$-Log-TV]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/g_zhu_mu0.07_alp200_u_28.3.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cam_20/g_zhu_mu0.07_alp200_f-u_20.5.jpg}
    \end{minipage}
    }    

    \subfigure[KR-TV]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/kr_lam2_alp200_u_27.4.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cam_20/kr_lam2_alp200_f-u_n_20.jpg}
    \end{minipage}
    }
    \subfigure[KR-Log-TV \eqref{kr_new_rel_log}]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/kr_zhu_a5_lam0.2_alp200_u_28.3.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/kr_zhu_a5_lam0.2_alp200_f-u_20.1.jpg}
    \end{minipage}
    }

    \subfigure[KR-Log-TV \eqref{KV-lip}]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/admm_kv_zhu_alp1e2_lam0.2_u_28.3.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/admm_kv_zhu_alp1e2_lam0.2_f-u_20.3.jpg}
    \end{minipage}
    }
    
    \caption{Results using the ROF model \eqref{rof}, $G$-TV model, and the KR-TV model \eqref{kr_new_rel}, compared with those models with Log-TV regularization \eqref{first}.
    The noisy image is corrupted by Gaussian noise with level $\sigma=20/255$. The parameters in models are tuned in order to satisfy the constraint $\|f-u\|_F \approx 20$.
    }
    \label{Fig:cam_20}
\end{figure}



==> KR_denoising/Experiment/grayscale/KR_Log_TV_1.tex <==
In Figure \ref{Fig:bar_2_15}, we consider a local part of the "Barbara" image with size $256 \times 256$.
The parameters are tuned so that the removed noise part has the norm $\|f-u\|_F \approx 15$ for all the models. 


Though the KR-TV model performs better in keeping the main contours in the $u$ component than ROF model, it cannot distinguish between noise and texture, since the KR-TV model \eqref{kr_new_rel} should constrast with the Vese and Osher's functional \eqref{VO} in the case $p=1$ \cite{vese2003modeling}.
The model \eqref{uvw} provides a solution of separating noise from texture.

The KR-Log-TV model leave less signal information in the residual image $f-u+100/255$ than the KR-TV model.
This is due to the fact that the use of the regularizer \eqref{first} helps keep large image gradient and thus preserves image contrasts.

As shown in the result $u$, the restored image by the KR-Log-TV model is brighter than the one by ROF in the white regions like the forehead, while the former is darker in the dark regions like the hair, which indicates that our model keeps more image contrasts. 

The $G$-TV model keeps more image contrasts than the ROF model.
The TV models present the staircase effect, while the KR-Log-TV model \eqref{kr_new_rel} generates more smooth image, which is mainly due to the employment of $L^2$-norm of gradient as a regularizer over the regions with relatively small image gradient.

%The model with Log-TV \eqref{first} preforms better in preserve image contrasts than 

\begin{figure}
%    \centering
    \flushright
    \subfigure[Original Image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_2/bar_2.eps}
    \end{minipage}
    }  
    \subfigure[ROF]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_2/rof_alp20_u_27.71.eps}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_2/rof_alp20_f-u.eps}
    \end{minipage}
    }
    
%    \subfigure[Log-TV]{
%        \begin{minipage}{0.3\linewidth}
%        \centering
%        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_2/zhu_alp8_a7_u_27.44.eps}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/255$]{
%        \begin{minipage}{0.3\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_2/zhu_alp8_a7_f-u_14.8.eps}
%    \end{minipage}
%    }
    \subfigure[Noisy Image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_2/bar_2_15.eps}
    \end{minipage}
    }    
    \subfigure[$G$-TV]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_2/g_alp100_mu3.3_u_28.21.eps}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_2/g_alp100_mu3.3_f-u_14.8.eps}
    \end{minipage}
    }
%    \subfigure[$G$-Log-TV]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/bar_2_ADMM/uv_g_zhu_a5_alp1e2_lam0.04_u_27.9.jpg}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/255$]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/bar_2_ADMM/uv_g_zhu_a5_alp1e2_lam0.04_f-u.jpg}
%    \end{minipage}
%    }
    
    \subfigure[KR-TV]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_2/kr_tv_alp200_lam3_u_27.43.eps}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_2/kr_tv_alp200_lam3_f-u_14.7.eps}
    \end{minipage}
    }
    
    \subfigure[KR-Log-TV]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_2/kr_zhu_a8_alp100_lam0.9_u_27.72.eps}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_2/kr_zhu_a8_alp100_lam0.9_f-u_14.5.eps}
    \end{minipage}
    }
    
    \caption{Results using the ROF model \eqref{rof}, $G$-TV \eqref{g-pro-l2}, and the proposed KR-TV model \eqref{kr_new_rel} with $\lambda=3,\alpha=200$ and KR-Log-TV model \eqref{kr_new_rel_log} with $a=8/255,\lambda=0.8,\alpha=100$. The noisy image is corrupted by Gaussian noise with level $\sigma=15/255$. 
    }
    \label{Fig:bar_2_15}
\end{figure}


%\begin{figure}
%    \centering
%     \subfigure[OSV]{
%        \begin{minipage}{0.3\linewidth}
%        \centering
%        \includegraphics[width= \linewidth]{KR_denoising/figure/eps/bar_2/osv_alp100_mu5.3_u_27.92.eps}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/255$]{
%        \begin{minipage}{0.3\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_2/osv_alp100_mu5.3_f-u_14.6.eps}
%    \end{minipage}
%    }
    
%    \subfigure[OSV-Log-TV]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/bar_2_ADMM/admm_osv_zhu_alp1e2_lam1e2_u_27.6.jpg}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/255$]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/zhu_TV/bar_2_ADMM/admm_osv_zhu_alp1e2_lam1e2_f-u_n_14.6.jpg}
%    \end{minipage}
%    }
%    \caption{Results using the OSV model \eqref{osv}.}
%    \label{fig:enter-label}
%\end{figure}

==> KR_denoising/Experiment/grayscale/KV_deblur.tex <==
In Figure \ref{Fig:blur}, we show deblurring results using the proposed model \eqref{KV-lip}.
Figure \ref{Fig:blur_noi} shows the cartoon + texture decomposition using the model \eqref{KV-lip} of deconvolution in the presence of noise, and a comparison with the RO model . 
The improvement of the proposed model over the RO model is noticed.
\begin{figure}
    \centering
    \subfigure[Blurry Image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/KV_model/bar_ave_7_0.jpg}
    \end{minipage}
    }
    \subfigure[RO model]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/KV_model/bar_ave_7_0_alp5e3_26.8.jpg}
    \end{minipage}
    }
    
    \subfigure[$\Delta g+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/bar_ave_7_0_kv_alp5e3_lam0.1_g.jpg}
    \end{minipage}
    }
    \subfigure[$u$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/bar_ave_7_0_kv_alp5e3_lam0.1_u.jpg}
    \end{minipage}
    }
    \subfigure[$u+\Delta g$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/bar_ave_7_0_kv_alp5e3_lam0.1_u+g_32.jpg}
    \end{minipage}
    }
    \caption{Deblurring results. Recovered texture parts $\Delta g+100/255$, cartoon $u$ and recovered images $u+\Delta g$ using the proposed model \eqref{KV-lip}, for a blurry image where a $7 \times 7$ averaging kernel was used using the model \eqref{KV-lip} with $\lambda=0.1$.}
    \label{Fig:blur}
\end{figure}



\begin{figure}
    \centering
    \subfigure[Blurry noisy image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/bar_1.75_11_1.15.jpg}
    \end{minipage}
    }
    \subfigure[ROF]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/bar_1.75_11_1.15_rof_alp2e3_24.4.jpg}
    \end{minipage}
    }
    
    \subfigure[$\Delta g+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/bar_1.75_11_1.15_kv_alp5e2_lam0.05_del_g.jpg}
    \end{minipage}
    }
    \subfigure[$u$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/bar_1.75_11_1.15_kv_alp5e2_lam0.05_u.jpg}
    \end{minipage}
    }
    \subfigure[$u+\Delta g$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/bar_1.75_11_1.15_kv_alp5e2_lam0.05_u+g_24.5.jpg}
    \end{minipage}
    }

    \subfigure[Original image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/man.jpg}
    \end{minipage}
    }
    \subfigure[Blurry noisy image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/man_1.75_11_1.15.jpg}
    \end{minipage}
    }
    \subfigure[ROF]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/man_1.75_11_1.15_rof_alp3e2_28.7.jpg}
    \end{minipage}
    }
    
    \subfigure[$\Delta g+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/man_1.75_11_1.15_kr_alp5e2_lam0.1_del_g.jpg}
    \end{minipage}
    }
    \subfigure[$u$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/man_1.75_11_1.15_kr_alp5e2_lam0.1_u.jpg}
    \end{minipage}
    }
    \subfigure[$u+\Delta g$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/man_1.75_11_1.15_kr_alp5e2_lam0.1_u+g_28.4.jpg}
    \end{minipage}
    }
    \caption{Restored using RO model. Recovered texture parts $\Delta g+100/255$, cartoon $u$ and recovered images $u+\Delta g$ using the proposed model \eqref{KV-lip}, for a noisy blurry image where a $11 \times 11$ Gaussian kernel standard deviation 1.75 was used and then noise of standard deviation 1.15 was added.}
    \label{Fig:blur_noi}
\end{figure}


==> KR_denoising/Experiment/grayscale/bab_35.tex <==
\subsection{A non-local algorithm for image denoising}
The paper \cite{nlm} propose to use the method noise $f-u$ to evaluate and compare the performance of digital image denoising methods and propose a new algorithm,
the non local means (NL-means). If a denoising method performs well, the method noise must look like a noise even with non noisy images and should contain as little structure as possible.

The human eye is the only one able to decide if the quality of the image has been improved by the denoising method, and the visual quality of the restored images, the non presence of artifacts and the correct reconstruction of edges, texture and details are compared.
This numerical measurement including the mean square error (MSE) is the most objective one. However, this error is not computable in a real problem and a small MSE
does not assure a high visual quality.

The primary scope of the $G$-TV model is not denoising since the oscillatory part contains both noise and texture.

In figure \ref{Fig:bab_rof} and \ref{Fig:bab_uvw}, the experiments are simulated by adding a gaussian
white noise of standard deviation $\sigma=35/255$ to the true image.
\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bab_35/bab.jpg}
    \end{minipage}
    }
    \subfigure[Noisy Image $f$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bab_35/bab_35.jpg}
    \end{minipage}
    }
    
    \subfigure[ROF $u$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bab_35/rof_alp8_u_23.2.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bab_35/rof_alp8_f-u_n_72.jpg}
    \end{minipage}
    }

    \subfigure[NL-means $u$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bab_35/nlm_h2_0.2_u_23.6.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bab_35/nlm_h2_0.2_f-u_n_63.jpg}
    \end{minipage}
    }

    \caption{Results using the ROF model for $\alpha=8$ and the NL-means \cite{nlm} for the noisy image (standard deviation 35).}
    \label{Fig:bab_rof}
\end{figure}


\begin{figure}
    \centering
    \subfigure[Model \eqref{uvw} $u$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bab_35/uvw_alp50_lam1_db8_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bab_35/uvw_alp50_lam1_db8_v.jpg}
    \end{minipage}
    }
    
    \subfigure[$u+v$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bab_35/uvw_alp50_lam1_db8_u+v_22.7.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bab_35/uvw_alp50_lam1_db8_f-u-v.jpg}
    \end{minipage}
    }

    \subfigure[Model \eqref{uvw} with DCT $u$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bab_35/uvw_lam1_dct_s_2_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bab_35/uvw_lam1_dct_s_2_v.jpg}
    \end{minipage}
    }
    
    \subfigure[$u+v$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bab_35/uvw_lam1_dct_s_2_u+v_22.9.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bab_35/uvw_lam1_dct_s_2_f-u-v_n_71.jpg}
    \end{minipage}
    }
    
    \caption{Results using the decomposition model \eqref{uvw}, for $\alpha=50,\lambda=1$, and the model \eqref{uvw} where $\|v\|_{B_{1,1}^1}$ is replaced by $\|\mathcal{D}v\|$, for $\alpha=100, \lambda=1, \delta=2\sigma$.}
    \label{Fig:bab_uvw}
\end{figure}


==> KR_denoising/Experiment/grayscale/barbara_1.tex <==
%\subsection{Modeling Textures with Total Variation Minimization and Oscillating Patterns in Image Processing}



We discuss the $u + v + w$ decompositions, with $u \in BV(\Omega)$ a cartoon component, $v=\mathrm{div}(m)$ an osillatory component, and $w$ a noise component, and study of separating noise from texture in section \ref{car-tex}.

In Figure \ref{Fig:dec}, we consider a real texture image without noise for the initial data $f$, and compare the image decomposition results using the ROF model \eqref{rof} and the proposed model \eqref{kr_new_rel}, for the same parameter $\alpha=30$. 

%We set the parameter $\lambda=0.5$ in \eqref{kr_new_rel}, and the parameters $\mu$ in\eqref{g-pro-l2} is tuned such that $\|v\|_{L^2}$ is almost the same as the proposed model. 

%The results obtained with the numerical approach for G-TV model are slightly better than the ones obtained with the ROF model \cite{2006Structure}.
%For the proposed model in the last row, there is less geometry in the texture image and the texture is separated \cite{2012Regularized}.

Note that in the residual $f-u-v$ by the proposed model, there is less geometry and texture than by the ROF model. The image $u$ is the cartoon part of $f$ while $v$ is the oscillations.

  \begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/bar_1.jpg}
    \end{minipage}
    }
    \subfigure[ROF]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_0/rof_u_alp30.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_0/rof_f-u_alp30.jpg}
    \end{minipage}
    }
    
    \subfigure[KR-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_0/kr_lam0.5_alp30_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_0/kr_lam0.5_alp30_v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_0/kr_lam0.5_alp30_u+v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_0/kr_lam0.5_alp30_f-u-v.jpg}
    \end{minipage}
    }  
    \caption{Image decomposition results using the ROF model with parameter $\alpha=30$, and the proposed model, for the same parameter $\alpha=30$. }
    \label{Fig:dec}
\end{figure}


==> KR_denoising/Experiment/grayscale/barbara_15.tex <==
In Figure \ref{Fig:barbara}, we show a real image and a noisy image $f$ with noise level $\sigma=15/255$. 
We show the result $u$ and the residual $f-u+100/255$ using the ROF model \eqref{rof} with parameter $\alpha$ in the second row.
The result $u$, $v$, $u+v$ and $f-u-v+100/255$ using the proposed model with $\lambda=2$ for the same parameter $\alpha$.
\begin{figure}
    \centering
    %\flushright
    \subfigure[$f$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_15/barbara.png}
    \end{minipage}
    }
    \subfigure[Noisy Image ($\sigma=15/255$)]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_15/bar_15.jpg}
    \end{minipage}
    }
    
    \subfigure[ROF]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_15/rof_u_alp20_27.38_0.807.jpg}
    \end{minipage}
    }
    \subfigure[ROF residual]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_15/rof_f-u_alp20.jpg}
    \end{minipage}
    }

    \subfigure[$u$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_15/kr_lam3_alp20_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_15/kr_lam3_alp20_v.jpg}
    \end{minipage}
    }

    \subfigure[$u+v$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_15/kr_lam3_alp20_u+v_27.7_0.786.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_15/kr_lam3_alp20_f-u-v.jpg}
    \end{minipage}
    }
    \caption{Results using the ROF model and the proposed model with $\lambda=3$, for the same parameter $\alpha=20$.}
    \label{Fig:barbara}
\end{figure}


In Figure \ref{Fig:barbara_osv}, we replace the norm $B^*(\frac{w}{\delta})$ in \eqref{uvw} with the norm in $H^{-1}(\Omega)$ \eqref{osv_norm} to model white Gaussian noise, and use the norm $\|v\|_{\mathrm{Lip}^*}$ to model texture.
\begin{figure}
    \centering
    \subfigure[OSV]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/OSV/bar_15_admm_kv_alp1e3_lam6e2_u_26.5.jpg}
    \end{minipage}
    }
    \subfigure[OSV residual]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/OSV/bar_15_admm_kv_alp1e3_lam6e2_f-u_n_33.5.jpg}
    \end{minipage}
    }
    
    \subfigure[$u$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/OSV/bar_15_alp5e2_kr_lam3_osv_lam6e2_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/OSV/bar_15_alp5e2_kr_lam3_osv_lam6e2_v.jpg}
    \end{minipage}
    }

    \subfigure[$u+v$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/OSV/bar_15_alp5e2_kr_lam3_osv_lam6e2_u+v_27.12.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/OSV/bar_15_alp5e2_kr_lam3_osv_lam6e2_f-u-v_n_30.jpg}
    \end{minipage}
    }
    \caption{Results using the OSV model \eqref{osv} and the model \eqref{uvw} with $H^{-1}$ norm for noise and $\|v\|_{\mathrm{Lip}^*}$ for texture.}
    \label{Fig:barbara_osv}
\end{figure}


==> KR_denoising/Experiment/grayscale/barbara_1_15.tex <==




In Figure \ref{Fig:bar_rof}, we consider a noisy image with noise level $\sigma=15/255$, and show the result $u$ and the residual $f-u+100/255$ using the ROF model \eqref{rof} with parameter $\alpha=20$.

\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/bar_1.jpg}
    \end{minipage}
    }
    \subfigure[Noisy Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/bar_1_15.jpg}
    \end{minipage}
    }
    \subfigure[ROF]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/rof_alp20_u_24.15_0.746.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/rof_alp20_f-u.jpg}
    \end{minipage}
    }

    \caption{Results using the ROF model with $\alpha=20$. }
    \label{Fig:bar_rof}
\end{figure}



In Figure \ref{Fig:bar_lip}, we show results obtained with the proposed model \eqref{kr_new_rel} for the same parameter $\alpha=20$ as the ROF model in Figure \ref{Fig:bar_rof}, for various $\lambda$. Note that, for decreasing $\lambda$, more texture appears in the $v$ component by the proposed model, but also more noise is kept.
  \begin{figure}
    \centering
    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam4_alp20_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam4_alp20_v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam4_alp20_u+v_24.53_0.767.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam4_alp20_f-u-v.jpg}
    \end{minipage}
    }

    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam3_alp20_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam3_alp20_v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam3_alp20_u+v_25.25_0.785.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam3_alp20_f-u-v.jpg}
    \end{minipage}
    }
    
    
    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam2_alp20_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam2_alp20_v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam2_alp20_u+v_26.01_0.783.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam2_alp20_f-u-v.jpg}
    \end{minipage}
    }
    %\subfigure[$u-f+100$]{
    %    \begin{minipage}{0.2\linewidth}
        %\caption{$u-f+100$}
    %    \centering
    %    \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/cartoon/fs_tv_bar_car_63200rof_res.jpg}
    %\end{minipage}
    %}

    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam1_alp20_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam1_alp20_v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam1_alp20_u+v_26.01_0.747.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/kr_lam1_alp20_f-u-v.jpg}
    \end{minipage}
    }

    \caption{Results using the proposed model with $\alpha=20$ and $\lambda=4,3,2,1$.}
    \label{Fig:bar_lip}
\end{figure}





==> KR_denoising/Experiment/grayscale/barbara_1_25.tex <==


In Figure \ref{Fig:bar_rof}, we consider a noisy image with noise level $\sigma=25/255$, and show the result $u$ and the residual $f-u+100/255$ using the ROF model \eqref{rof} with parameter $\alpha=10$.

\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/bar_1.jpg}
    \end{minipage}
    }
    \subfigure[$f$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/bar_1_25.jpg}
    \end{minipage}
    }
    \subfigure[ROF $u$ 22.2]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/u_rof_alp10_21.3.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/f-u_rof_alp10_n_31.jpg}
    \end{minipage}
    }

    \caption{Results using the ROF model with $\alpha=10$.}
    \label{Fig:bar_rof}
\end{figure}



In Figure \ref{Fig:bar_1_25}, we show results obtained with the proposed model \eqref{kr_new_rel} for various $\lambda$, but the same parameter $\alpha=10$. 
Note that, for decreasing $\lambda$, more texture appears in the $v$ component by the proposed model, but also more noise is kept.
For smaller $\lambda$, both the texture and the noise are kept in the $v$ component and therefore in the sum $u+v$.
  \begin{figure}
    \centering
       \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam4/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam4/v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam4/u+v_21.7.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam4/f-u-v_n_28.5.jpg}
    \end{minipage}
    }
    
    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam3/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam3/v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam3/u+v_22.27.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam3/f-u-v_n_25.7.jpg}
    \end{minipage}
    }

    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam2/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam2/v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam2/u+v_22.8.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam2/f-u-v_n_21.jpg}
    \end{minipage}
    }

    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam0.5/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam0.5/v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam0.5/u+v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam0.5/f-u-v.jpg}
    \end{minipage}
    }
    
    \caption{Results using the proposed model \eqref{kr_new_rel} with $\alpha=10$ and $\lambda=4,3,2,0.5$.}
    \label{Fig:bar_1_25}
\end{figure}







==> KR_denoising/Experiment/grayscale/barbara_25.tex <==
In Figure \ref{Fig:09_uv}, the noisy image is corrupted by Gaussian noise with level $\sigma=25/255$, and the additive noise $n$ has the Frobenius norm $\|n\|_F = N\|n\|_{F'} = N \sigma$.
The removed noise part has the norm $\|f-u\|_F = N\|f-u\|_{F'} \approx 50 = N\sigma$.

\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_15/barbara.png}
    \end{minipage}
    }
    \subfigure[Noisy Image $f$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara/09_25.jpg}
    \end{minipage}
    }
    
    \subfigure[ROF $u$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara/rof_alp13_u_25.4.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara/rof_alp13_f-u_n_49.jpg}
    \end{minipage}
    }

    \subfigure[KR-$L^2$-TV $u$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/alp10_lam3/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/alp10_lam3/v.jpg}
    \end{minipage}
    }
    
    \subfigure[$u+v$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/alp10_lam3/u+v_25.0.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/alp10_lam3/f-u-v_n_48.jpg}
    \end{minipage}
    }

    \caption{Results using the ROF model for $\alpha=13$, and the proposed model \eqref{kr_new_rel} for $\alpha=10,\lambda=3$. The removed noise part has the norm $\|f-u-v\|_F \approx 50$ for the proposed model. }
    \label{Fig:09_uv}
\end{figure}






\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/bar.jpg}
    \end{minipage}
    }
    \subfigure[$f$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/bar_2_25.jpg}
    \end{minipage}
    }
    \subfigure[ROF $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/rof_alp12_u_25.4.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/rof_alp12_f-u_n_24.5.jpg}
    \end{minipage}
    }

    \subfigure[KR-$L^2$-TV \eqref{kr_new_rel} $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/alp10_lam3/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/alp10_lam3/v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/alp10_lam3/u+v_24.7.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/alp10_lam3/f-u-v_n_24.jpg}
    \end{minipage}
    }
    \caption{Results using the ROF model with $\alpha=12$, the KR-$L^2$-TV \eqref{kr_new_rel}, for $\alpha=10, \lambda=3$.}
    \label{Fig:bar_2_uv}
\end{figure}

==> KR_denoising/Experiment/grayscale/barbara_2_15.tex <==
Note that the proposed model \eqref{kr_new_rel} is the same as the Vese and Osher's functional \eqref{VO} for solving the G-TV model in the case $p=1$. Therefore, we show the numerical results similar to those in \cite{vese2003modeling}.


Figure \ref{Fig:car_bar_2} shows a comparison between the proposed models \eqref{kr_new_rel} and \eqref{KV-Jung} with the ROF model and the G-TV model.

\begin{figure}
    \centering
    \subfigure[$f$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/bar.jpg}
    \end{minipage}
    }

    \subfigure[ROF $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2/rof_alp13_1.56e3_u.jpg}
    \end{minipage}
    }
    \subfigure[G-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2/g_tv_alp100_1.55e4_u.jpg}
    \end{minipage}
    }
    \subfigure[KR-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2/kr_lam1_alp2e2_u_1.52e3.jpg}
    \end{minipage}
    }
    \subfigure[W-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2/W_tv_FS_1.54e3_u.jpg}
    \end{minipage}
    }

    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2/rof_alp13_1.56e3_f-u.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2/g_tv_alp200_mu0.06_f-u.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2/kr_lam1_alp2e2_f-u.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2/W_tv_FS_1.54e3_f-u.jpg}
    \end{minipage}
    }
    \caption{$f$ is a given image to be decomposed. The first image decomposition results $u$ and $f-u+100/255$ is obtained using the ROF model.
    The second decomposition is obtained by \eqref{g-pro-l2} for the $G$-TV model \cite{2005Image}. 
    The third decomposition is obtained by the proposed model \eqref{kr_new_rel} solved by algorithm in section \ref{alg-kr}. 
    The fourth results is obtained by W-TV \cite{2015A}.
    For the G-TV model and the proposed model, we use the same parameter $\alpha=200$. The parameters are chosen such that the total variations of the cartoon part of the these methods are almost the same.
    We can notice the improvement from left to right in terms of cartoon and texture decomposition.}
    \label{Fig:car_bar_2}
\end{figure}




In Figure \ref{Fig:uv}, we consider the noisy image with noise level $\sigma=15/255$, and show the result $u$ and the residual using the ROF model parameter $\alpha=20$ in the first row. 
Then we show results obtained with the proposed model for the same parameter $\alpha=20$ and various $\lambda$. 
Note that, for decreasing $\lambda$, more texture appears in the $v$ component by the new model, but also more noise is kept.

  \begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/bar.jpg}
    \end{minipage}
    }
    \subfigure[Noisy Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/bar_15.jpg}
    \end{minipage}
    }
    \subfigure[ROF]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/alp20_rof_27.68_0.820.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/alp20_rof_f-u.jpg}
    \end{minipage}
    }
    
    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/u_lam3.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/v_lam3.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/u+v_lam3._27.42_0.972jpg.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/f-u-v_lam3.jpg}
    \end{minipage}
    }
    
    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/u_lam2.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/v_lam2.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/u+v_lam2.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/f-u-v_lam2.jpg}
    \end{minipage}
    }
    %\subfigure[$u-f+100$]{
    %    \begin{minipage}{0.2\linewidth}
        %\caption{$u-f+100$}
    %    \centering
    %    \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/cartoon/fs_tv_bar_car_63200rof_res.jpg}
    %\end{minipage}
    %}

    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/u_lam1.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/v_lam1.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/u+v_lam1.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/f-u-v_lam1.jpg}
    \end{minipage}
    }
    
    \caption{Results using the ROF model with $\alpha=20$ and the proposed model with $\alpha=20$ and $\lambda=3,2,1$. }
    \label{Fig:uv}
\end{figure}





==> KR_denoising/Experiment/grayscale/bregman.tex <==
\subsection{Bregman iterative regularization}

{\color{red}Is this subsection related to our models and algorithms? If not, we can remove it.}

%The models related to Meyer's $G$-TV Model performs well to separate cartoon from texture which can be used to improve image inpainting algorithms \cite{inpainting}.
Osher et al. \cite{bregman} proposed a new iterative regularization procedure for image restoration problems based on the use of Bregman distances, which appear to give significant improvement over ROF model for denoising.

Instead of solving the ROF model \eqref{rof} once, the Bregman iterative regularization procedure of Osher et. al. \cite{bregman} solves a sequence of convex problems
\begin{enumerate}
    \item initialize: $u_0=0$ and $v_0=0$.
    \item For $k=0,1,2,\cdots$: compute $u_{k+1}$ by solving
    $u_{k+1} = \mathrm{arg}\min_u J(u) - J(u_k) - \langle v_k, u-u_k \rangle + \frac{\alpha}{2}\|u-f\|^2$, which is a minimizer of the modified ROF model, 
    \begin{equation}
        u^{k+1} = \mathrm{arg}\min_u J(u) + \frac{\alpha}{2}\|u-f-v_k\|^2
    \end{equation}
    and update
    \begin{equation}
        v_{k+1} = v_k + f - u_{k+1}.
    \end{equation}
\end{enumerate}
The stopping rule is stopping the iterative procedure the first time the residual $\|u_k - f\|_{L^2} < \sigma$.
The numerical results for denoising appear to give significant improvement over ROF model.

In \cite{bregman}, the above regularization procedure generalizes to the Vese and Osher's functional \eqref{VO},
\begin{enumerate}
    \item initialize: $u_0=0$ and $w_0=0$.
    \item For $k=0,1,2,\cdots$: compute $u_{k+1}$ and $m_{k+1}$ as a minimizer of the model, 
    \begin{equation}
    \inf_{(u,m)} \int_{\Omega} |\nabla u| + \frac{\alpha}{2} \int_{\Omega}|f + w_k - u - \mathrm{div}(m)|^2 + \lambda [ \int_{\Omega} ( \sqrt{m_1^2 + m_2^2} )^p ]^{\frac{1}{p}},
    \end{equation}
    and update
    \begin{equation}
        w_{k+1} = w_k + f - u_{k+1} - \mathrm{div}(m_{k+1}).
    \end{equation}
\end{enumerate}

\begin{figure}
    \centering
    \subfigure[ROF with iterative regularization]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_2/bregman/bregman_u_27.52.eps}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_2/bregman/bregman_f-u_14.7.eps}
    \end{minipage}
    }
    
    \subfigure[KR-TV with iterative regularization]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_2/bregman/breg_kr_alp1_lam3_u_27.57.eps}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/eps/bar_2/bregman/breg_kr_alp1_lam3_f-u_14.9.eps}
    \end{minipage}
    }
    \caption{Results using the ROF with iterative regularization with $\alpha=1$, and the KR-TV with iterative regularization with $\lambda=3$ and $\alpha=1$, for noise level $\sigma=15/255$.
    }
    \label{Fig:bre_bar}
\end{figure}


%Osher et al. \cite{bregman} proposed a new iterative regularization procedure for image restoration problems based on the use of Bregman distances.
%The numerical results for denoising of textured images appear to give significant improvement over the ROF model.
%The Bregman iterative procedure stops in the first time the residual $\|f-u_k\|^2_{L^2} \leq \sigma^2$.
%\begin{figure}
%    \centering
%    \subfigure[Model \cite{bregman} $u$ 27.3]{
%    \begin{minipage}{0.3\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/Bregman/barbara_15/lam1_ite13_27.3.jpg}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/25$]{
%        \begin{minipage}{0.3\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/Bregman/barbara_15/lam1_ite13_f-u_n_30.jpg}
%    \end{minipage}
%    }
%    \caption{The result is obtained by the iterative regularization with ROF in \cite{bregman}.}
%    \label{fig:bregman}
%\end{figure}

==> KR_denoising/Experiment/grayscale/cam_20.tex <==
In Figure \ref{Fig:cam_20}, we apply our model to a real image "Cameraman".
For $G$-TV model \eqref{g-pro-l2} and the KR-Log-TV model \eqref{kr_new_rel_log}, we set $\alpha=50$ and the other parameters in the models are tuned in order to satisfy the constraint $\|f-u\|_F \approx 20$.
From the residual images $f-u+100/255$, we can see that more meaningful signals are removed as noise by the ROF model than by the KR-Log-TV model, which indicate that the KR-Log-TV model preserve the image contrast better. 
\begin{figure}
%    \centering
    \flushright
    \subfigure[Original Image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/01.png}
    \end{minipage}
    }
    \subfigure[ROF]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/rof_u_alp14_28.4.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/rof_u_f-u_n_19.9.jpg}
    \end{minipage}
    }    
%    \subfigure[$L^2$-Log-TV]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/zhu_a7_u_28.07.jpg}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/255$]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cam_20/zhu_a7_f-u_20.5.jpg}
%    \end{minipage}
%    }

    \subfigure[Noisy Image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/cam_20.jpg}
    \end{minipage}
    }    
    \subfigure[$G$-TV]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/g_mu0.05_alp50_u_28.33.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cam_20/g_mu0.05_alp50_f-u_20.5.jpg}
    \end{minipage}
    }
%    \subfigure[$G$-Log-TV]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        %\caption{Sink-TV}
%        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/g_zhu_a7_mu0.06_alp50_u_28.37.jpg}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/255$]{
%        \begin{minipage}{0.23\linewidth}
%        %\caption{FS-TV}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cam_20/g_zhu_a7_mu0.06_alp50_f-u_20.5.jpg}
%    \end{minipage}
%    }    

    \subfigure[OSV]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/osv_alp50_lam350_u_28.22.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cam_20/osv_alp50_lam350_f-u_20.2.jpg}
    \end{minipage}
    }
%    \subfigure[OSV-Log-TV]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/osv_zhu_a7_alp50_lam100_u_28.38.jpg}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/255$]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cam_20/osv_zhu_a7_alp50_lam100_f-u_20.1.jpg}
%    \end{minipage}
%    }  
    
%    \subfigure[KR-TV]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/kr_alp50_lam2.5_u_27.62.jpg}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/255$]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/cam_20/kr_alp50_lam2.5_f-u_20.jpg}
%    \end{minipage}
%    }
    \subfigure[KR-Log-TV \eqref{kr_new_rel_log}]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/kr_zhu_a7_alp50_lam0.04_u_28.03.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/kr_zhu_a7_alp50_lam0.04_f-u_20.4.jpg}
    \end{minipage}
    }

%    \subfigure[KR-Log-TV \eqref{KV-lip}]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/admm_kv_zhu_alp1e2_lam0.2_u_28.3.jpg}
%    \end{minipage}
%    }
%    \subfigure[$f-u+100/255$]{
%        \begin{minipage}{0.23\linewidth}
%        \centering
%        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/cam_20/admm_kv_zhu_alp1e2_lam0.2_f-u_20.3.jpg}
%    \end{minipage}
%    }
    
    \caption{Results using the ROF model \eqref{rof}, $G$-TV model \eqref{g-pro-l2}, OSV model \eqref{osv} and the KR-Log-TV model \eqref{kr_new_rel_log}.
    The noisy image is corrupted by Gaussian noise with level $\sigma=20/255$. 
    }
    \label{Fig:cam_20}
\end{figure}

==> KR_denoising/Experiment/grayscale/inpainting.tex <==
For the model \eqref{KV-lip} under the assumption that the image $f$ has a missing region, denoted by $T \in \Omega$. 
We can define $S = \mathbf{I}_{T}$ and the model is rewritten as 
\begin{equation}
    \inf_{(u,v)\in BV\times H} \mathrm{TV}(u) + \frac{\alpha}{2} \int_{\Omega} |\mathbf{I}_{T}(f-K*(u+v))|^2 dx + \lambda \|v\|_{\mathrm{Lip}^*}.
\end{equation}

In Figure \ref{Fig:bar_inp},

\begin{figure}
    \centering
    \subfigure[]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/inpainting/bar_0.5.jpg}
    \end{minipage}
    }
    \subfigure[$L^2$-TV $u$ 25.8]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/inpainting/bar_0.5_rof_alp50_u_25.78.jpg}
    \end{minipage}
    }
    
    \subfigure[Model \eqref{KV-lip} $u$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/inpainting/bar_0.5_KV_ADMM_lam25_beta2_u.jpg}
    \end{minipage}
    }
    \subfigure[$\Delta g + 100/25$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/inpainting/bar_0.5_KV_ADMM_lam25_beta2_del_g.jpg}
    \end{minipage}
    }
    \subfigure[$u+\Delta g$ 25.3]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/KV_model/inpainting/bar_0.5_KV_ADMM_lam25_beta2_u+del_g_25.3.jpg}
    \end{minipage}
    }
    
    \caption{Inpainting and decomposition results of the ROF model with $\alpha=50$ and the model \eqref{KV-lip}, for $\alpha=50,\lambda=2$.}
    \label{Fig:bar_inp}
\end{figure}





==> KR_denoising/Experiment/grayscale/log_tv.tex <==
\subsection{Log-TV}
In \cite{zhu}, the author employ the averaged Frobenius norm $\|f\|_{F'} = \frac{\|f\|_{F}}{N} = \sqrt{\sum_{i=1}^N \sum_{j=1}^N |f_{ij}|^2} / N$ to measure the removed noise part, and choose the regularization parameters for the proposed model and the ROF model so that their removed noise parts $\|f-u\|_{F'} \approx \sigma$ are almost the same.

In Figure \ref{Fig:u_n}, we show the result $u$ and the residual using the ROF model parameter $\alpha=1/20$ in the first row. 
Then we show results obtained with the proposed model for various $\alpha$.
The $256 \times 256$ noisy image is corrupted by Gaussian noise with level $\sigma=15/255$, and the additive noise $n$ has the Frobenius norm $\|n\|_F = 15.0$.
The parameters $\lambda$ are tuned such that the removed noise part has the norm $\|f-u\|_F \approx 15$ for both ROF and the proposed models. 

  \begin{figure}
    \centering
    \subfigure[ROF]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/rof_alp20_u_27.67.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/rof_alp20_f-u_n_14.9.jpg}
    \end{minipage}
    }
    \subfigure[KR-TV(ALM)]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/ALM_kr_beta0.4_u_26.9.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{KR TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/ALM_kr_beta0.4_f-u_n_15.1.jpg}
    \end{minipage}
    }
    
    \subfigure[$u$ ($\alpha=1/20$)]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp20_lam4_u_27.2.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp20_lam4_v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp20_lam4_f-u-v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp20_lam4_f-u_n_15.8.jpg}
    \end{minipage}
    }
    
    \subfigure[$u$ ($\alpha=1/30$)]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp30_lam3_u_27.4.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp30_lam3_v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp30_lam3_f-u-v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp30_lam3_f-u_n_15.3.jpg}
    \end{minipage}
    }
    %\subfigure[$u-f+100$]{
    %    \begin{minipage}{0.2\linewidth}
        %\caption{$u-f+100$}
    %    \centering
    %    \includegraphics[width= \linewidth]{KR_denoising/figure/ALM_KR/cartoon/fs_tv_bar_car_63200rof_res.jpg}
    %\end{minipage}
    %}

    \subfigure[$u$ ($\alpha=1/40$)]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp40_lam3_u_27.6.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp30_lam3_v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp40_lam3_f-u-v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15/kr_alp40_lam3_f-u_n_14.7.jpg}
    \end{minipage}
    }    
    \caption{Results using the ROF model for parameter $\alpha=0.05$ and the proposed model for parameters $\alpha=1/20,1/30,1/40$. The additive noise $n$ has the Frobenius norm $\|n\|_F = 15.0$ and the parameters $\lambda=4,3,3$ are tuned such that the removed noise parts have the norm $\|f-u\|_F \approx 15$ for the proposed models. }
    \label{Fig:u_n}
\end{figure}



We consider the first order regularization term $R(u) = \phi_a(\nabla u),\;a>0$ proposed in \cite{zhu,2023A} in \cite{2023A} for solving \eqref{upro-vomt}, where $\phi_a$ is defined as 
    \begin{equation}\label{first}
    \begin{split}
    \phi_a(x) = \left \{
        \begin{array}{lr}
            \frac{1}{2a} x^2,                 & |x|\leq a,\\
            a \ln |x| + \frac{a}{2} - a\ln a, & |x|> a,
        \end{array}
        \right.	
    \end{split}
    \end{equation}
The result using $u^{-1}=0$ and $u^{-1}=f$ are different which may due to the regularizer is non-convex.

In Figure \ref{Fig:log_uv}, we compare the Log-TV model \cite{2023A} and the proposed model using the Log-TV for solving the $\vec{u}$ subproblem \eqref{pro1}, for different $(\alpha,\lambda)$.
\begin{figure}
    \centering
    \subfigure[Log-TV $u$ 27.9]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/zhu_alp10_a0.15_h0.2_u_27.9.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/zhu_alp10_a0.15_h0.2_f-u.jpg}
    \end{minipage}
    }
    
    \subfigure[KR-Log-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp10_a0.15_h0.2_lam1_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp10_a0.15_h0.2_lam1_v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp10_a0.15_h0.2_lam1_u+v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp10_a0.15_h0.2_lam1_f-u-v.jpg}
    \end{minipage}
    }  
    
    \subfigure[KR-Log-TV $u$ 27.2]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp10_a0.15_h0.2_lam3_u_27.2.jpg}
    \end{minipage}
    }
    \subfigure[$v$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp10_a0.15_h0.2_lam3_v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$ 27.7]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp10_a0.15_h0.2_lam3_u+v_27.7.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp10_a0.15_h0.2_lam3_f-u-v.jpg}
    \end{minipage}
    }
    
    \subfigure[KR-Log-TV $u$ 27.7]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp20_a0.15_h0.2_lam1_u_27.77.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp20_a0.15_h0.2_lam1_v.jpg}
    \end{minipage}
    }  
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp20_a0.15_h0.2_lam1_u+v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/log_TV/kr_zhu_alp20_a0.15_h0.2_lam1_f-u-v.jpg}
    \end{minipage}
    }  
    \caption{Results using the Log-TV model \cite{2023A} for $h=0.2,a=0.15,\alpha=10$ and the proposed model using the Log-TV for solving the $\vec{u}$ subproblem \eqref{pro1}, for $(\alpha,\lambda)=(10,1),(10,3),(20,1)$.}
    \label{Fig:log_uv}
\end{figure}



In Figure \ref{Fig:log_n}, we compare the Log-TV model \cite{2023A} and the proposed model using the Log-TV for solving the $\vec{u}$ subproblem \eqref{pro1}, for different $\alpha$.
The the noisy image is corrupted by Gaussian noise with level $\sigma=15/255$, and the additive noise $n$ has the Frobenius norm $\|n\|_F = 15.0$.
The parameters $\lambda$ are tuned such that $\|f-u\|_F \approx 15$. 
\begin{figure}
    \centering
    \subfigure[Log-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/zhu_alp10_u_27.6.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/zhu_alp10_f-u_n_14.jpg}
    \end{minipage}
    }
    
    \subfigure[KR-Log-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp10_lam3_u_27.4.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp10_lam3_v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp10_lam3_f-u-v.jpg}
    \end{minipage}
    }  
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp10_lam3_f-u_n_14.7.jpg}
    \end{minipage}
    }
    
    \subfigure[KR-Log-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp20_lam1_u_27.6.jpg}
    \end{minipage}
    }
    \subfigure[$v$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp20_lam1_v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp20_lam1_f-u-v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp20_lam1_f-u_n_13.9.jpg}
    \end{minipage}
    }
    
    \subfigure[KR-Log-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp30_lam0.7_u_27.3.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp30_lam0.7_v.jpg}
    \end{minipage}
    }  
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp30_lam0.7_f-u-v.jpg}
    \end{minipage}
    }  
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/barbara_2_15_log_TV_h0.2_a0.15/kr_alp30_lam0.7_f-u_n_14.7.jpg}
    \end{minipage}
    }
    
    \caption{Results using the Log-TV model \cite{2023A} for $h=0.2,a=0.15,\alpha=10$ and the proposed model using the Log-TV for solving the $\vec{u}$ subproblem \eqref{pro1}, for $\alpha=1/10,1/20,1/30$.}
    \label{Fig:log_n}
\end{figure}

==> KR_denoising/Experiment/grayscale/uvw.tex <==
\subsection{$u+v+w$ Model}
In \cite{aujol2005dual}, Aujol et al. propose a decomposition model which splits an image into three components: a first one containing the structure of the image, a second one the texture of the image, and a third one the noise.
    \begin{equation}\label{uvw}
        \inf_{u,v,w} F(u,v,w) = \mathrm{TV}(u) + \lambda J^*(v) + B^*(\frac{w}{\delta}) + \frac{\alpha}{2}\|f-u-v-w\|^2,
    \end{equation} 
where three different norms are used: the total variation for the geometrical component, a negative Sobolev norm for the texture, and a negative Besov norm $B^*$ for the noise. 

In Meyer's $G$-TV model \eqref{g-pro}, negative Sobolev norms have seemed to be useful to modelize oscillating patterns.
The discrete version of a Sobolev norm ($p \geq 1$) is
\begin{equation}
    \|u\|_{1,p} = \|\nabla u\|_p = (\sum_{1\leq i,j \leq N} \|\nabla u_{i,j}\|_p)^{1/p}
\end{equation}
This is a norm on the space $G = \{u \in V: \sum_{i,j}u_{i,j} = 0\}$ and the negative Sobolev norm (with $1/p + 1/q = 1$) is
\begin{equation}\label{neg}
    \|v\|_{-1,p} = \sup_{\|u\|_{1,q}=1}(v,u) = \sup_{\|\nabla u\|_{q}=1}(v,u)
\end{equation}
The $G$ norm can be written as $\|v\|_G = \sup_{\|\nabla u\|_{1}=1}(v,u)$ \cite{2005Image}.
Osher, Sole and Vese (OSV) proposed a approximated model using the $\|\cdot\|_{-1,2}$.

The negative Besov norm (which amounts to a wavelet shrinkage) is adapted to the noise.
Given an orthonormal wavelet basis $\phi_{j}(x)$, the wavelet transform of an image $v$ is represented as $v = \sum_j \langle v, \phi_{j}\rangle \phi_{j}$.
Consider the Besov space $B^{1,1}_1(\Omega)$, the norm in $B^{1,1}_1(\Omega)$ is equivalent to $B(v) = \|v\|_{B^{1,1}_1}=\sum_j c_{j}$ where $c_{j}$ are the wavelet coefficients of $v$.

The convex functional \eqref{uvw} can be solved by minimization with respect to each of the variable $u,v$ and $w$ alternatively, i.e.,
\begin{itemize}
    \item $u,w$ being fixed, we search for $v$ as a solution of
    \begin{equation}\label{subv}
        \inf_v \frac{\alpha}{2} \int_{\Omega} |f-u-v-w|^2 dx + J^*(\frac{v}{\mu}), 
    \end{equation}
    
    \item $v,w$ being fixed, we search for $u$ as a solution of
    \begin{equation}\label{subu}
        \inf_{u} J(u) + \frac{\alpha}{2} \int_{\Omega} |f-u-v-w|^2 dx.
    \end{equation}

    \item $u,v$ being fixed, we search for $w$ as a solution of
    \begin{equation}\label{subw}
        \inf_w B^*(\frac{w}{\delta}) + \frac{\alpha}{2}\|f-u-v-w\|^2,
    \end{equation} 
\end{itemize}

\begin{proposition}[cf. Jean-Fran{\c{c}}ois Aujol \& Antonin Chambolle \cite{aujol2005dual}]\label{dual-norm}
Let $F$ be a convex function. Then the two following statements are equivalent:
\begin{itemize}
    \item $\hat{u}$ is a solution of
\begin{equation}
    \inf_u \left\{ F(u) + \frac{\alpha}{2}\|f-u\|^2 \right\},
\end{equation}
    \item $\hat{w} = f - \hat{u}$ is a solution of 
\begin{equation}
    \inf_w \left\{ F^*(\alpha w) + \frac{\alpha}{2}\|f-w\|^2. \right\}
\end{equation}
\end{itemize}
\end{proposition}

The minimization \eqref{subv} can be solved by using the Proposition \ref{dual-norm}, which states that $\hat{v}$ is a solution of \eqref{subv}, if and only if, $\hat{z} = f-u-w - \hat{v}$ is a solution of
    \begin{equation}\label{subv-1}
        \inf_{z} J(z) + \frac{1}{2\mu} \int_{\Omega} |f-u-w - z|^2 dx.
    \end{equation}
    
The two minimization problems \eqref{subu} and \eqref{subv-1} are almost the same as the traditional ROF model \eqref{rof}.
The dual problem of \eqref{subw} is
\begin{equation}\label{subw-d}
     \frac{1}{2}\|f-u-v-z\|^2 + \delta B(z),
\end{equation}
The solution of this problem $\hat{z}$ is obtained by a wavelet soft-thresholding algorithm with threshold $\delta$, and by Proposition \ref{dual-norm}, the solution of \eqref{subw} is $\hat{w} = (f-u-v)-\hat{z}$.

The parameter $\alpha$ controls the $L^2$ norm of the residual $f-u-v-w$ and $\delta = \eta \sigma \sqrt{2\log N^2}$ is the threshold which is used in the wavelet thresholding.

%If $F(u) = B^*(\frac{u}{\delta})$, then $F^*(w) = \delta \|\hat{w}\|_{B_{1,1}^1}$.

%If $F(u)=\|u\|_{-1,p}$ defined on the space $G$ \eqref{g-spa-dis}, which is the discrete norm for negative Sobolev spaces (with $\frac{1}{p} + \frac{1}{q} = 1$):
%\begin{equation}
%    \|u\|_{-1,p} = \sup_{\|\nabla v\|_{q}=1} \langle u,v\rangle,
%\end{equation}
%then $F^*(w)=\mathbf{I}_{\|\nabla w\|_{q}\leq 1}(w)$.

The norm $\|v\|_{\mathrm{Lip}^*}$ \eqref{lip} is the same as the negative Sobolev norm \eqref{neg} for $p=1$, and the $G$ norm is approximated by another negative Sobolev norm \eqref{sob} in the Osher and Vese’s functional \eqref{VO}.

We replace $J^*(v)$ by $\|v\|_{\mathrm{Lip}^*}$.
In Figure \ref{Fig:uvw}, and show the results of the model \eqref{uvw} with $\|v\|_{\mathrm{Lip}^*}$.
\begin{figure}
    \centering
    \subfigure[$u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/uvw/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/uvw/v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/uvw/u+v_lam2_27.71_0.814.jpg}
    \end{minipage}
    }
    \subfigure[$w+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_15/uvw/w.jpg}
    \end{minipage}
    }
    \caption{Results using the decomposition model \eqref{uvw}. The noisy image is corrupted by Gaussian noise with level $\sigma=15/255$.}
    \label{Fig:uvw}
\end{figure}


In Figure \ref{Fig:09_rof} and \ref{Fig:09_uvw}, the noisy image is corrupted by Gaussian noise with level $\sigma=25/255$, and the additive noise $n$ has the Frobenius norm $\|n\|_F = N\|n\|_{F'} = N \sigma$.
The removed noise part has the norm $\|f-u\|_F = N\|f-u\|_{F'} \approx 50 = N\sigma$.
\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_15/barbara.png}
    \end{minipage}
    }
    \subfigure[Noisy Image $f$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara/09_25.jpg}
    \end{minipage}
    }
    
    \subfigure[ROF $u$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara/rof_alp13_u_25.4.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.3\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara/rof_alp13_f-u_n_49.jpg}
    \end{minipage}
    }

    \caption{Results using the ROF model for $\alpha=13$. }
    \label{Fig:09_rof}
\end{figure}


\begin{figure}
    \centering
    \subfigure[KR-$L^2$-TV $u$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/alp10_lam3/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/alp10_lam3/v.jpg}
    \end{minipage}
    }
    
    \subfigure[$u+v$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/alp10_lam3/u+v_25.0.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/alp10_lam3/f-u-v_n_48.jpg}
    \end{minipage}
    }

    \subfigure[Model \eqref{uvw} $u$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/uvw/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/uvw/v_lam2.jpg}
    \end{minipage}
    }
    
    \subfigure[$u+v$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/uvw/u+v_lam2.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara/uvw/f-u-v_lam2_n_48.5.jpg}
    \end{minipage}
    }
    
    \caption{Results using the proposed model \eqref{kr_new_rel} for $\alpha=10,\lambda=3$, and the decomposition model \eqref{uvw}, for $\alpha=100,\lambda=2$. The removed noise part has the norm $\|f-u-v\|_F \approx 50$ for both the proposed model and the decomposition model.}
    \label{Fig:09_uvw}
\end{figure}



In Figure \ref{Fig:bar_1_rof} and \ref{Fig:bar_1_uvw}, the $512 \times 512$ image is corrupted by Gaussian noise with level $\sigma=25/255$, and the additive noise $n$ has the Frobenius norm $\|n\|_F = 25.0$.

\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/barbara_1_15/bar_1.jpg}
    \end{minipage}
    }
    \subfigure[$f$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/bar_1_25.jpg}
    \end{minipage}
    }
    \subfigure[ROF $u$ 22.2]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/u_rof_alp13_22.2.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{Sink-TV}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/f-u_rof_alp13_n_27.jpg}
    \end{minipage}
    }

    \caption{Results using the ROF model for $\alpha=13$. The removed noise part has the norm $\|f-u\|_F = 27$.}
    \label{Fig:bar_1_rof}
\end{figure}


\begin{figure}
    \centering
    \subfigure[KR-$L^2$-TV $u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam3/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam3/v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$ 22.3]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam3/u+v_22.27.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/alp10_lam3/f-u-v_n_25.7.jpg}
    \end{minipage}
    }

    \subfigure[Model \eqref{uvw} $u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/uvw/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/uvw/v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$ 23.3]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/uvw/u+v_23.3.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/uvw/f-u-v_n_25.jpg}
    \end{minipage}
    }
    
    \caption{Results using the proposed model \eqref{kr_new_rel} for $\alpha=10,\lambda=3$, and the decomposition model \eqref{uvw}, for $\alpha=100,\lambda=2$. The removed noise part has the norm $\|f-u-v\|_F \approx 25$ for both the proposed model and the model \eqref{uvw}.}
    \label{Fig:bar_1_uvw}
\end{figure}



\begin{figure}
    \centering
    \subfigure[Original Image]{
        \begin{minipage}{0.23\linewidth}
        \centering
        %\caption{ROF}
        \includegraphics[width= \linewidth]{KR_denoising/figure/new_model/bar_15/kr_l2_tv_alp0.05/bar.jpg}
    \end{minipage}
    }
    \subfigure[$f$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/bar_2_25.jpg}
    \end{minipage}
    }
    \subfigure[ROF $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/rof_alp12_u_25.4.jpg}
    \end{minipage}
    }
    \subfigure[$f-u+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/rof_alp12_f-u_n_24.5.jpg}
    \end{minipage}
    }

    \subfigure[KR-$L^2$-TV \eqref{kr_new_rel} $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/alp10_lam3/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/alp10_lam3/v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/alp10_lam3/u+v_24.7.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/alp10_lam3/f-u-v_n_24.jpg}
    \end{minipage}
    }

    \subfigure[Model \eqref{uvw} $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw/u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw/v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw/u+v.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw/f-u-v_n_24.jpg}
    \end{minipage}
    }
  
    \subfigure[Model \eqref{uvw} with DCT $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw_dct/uvw_lam1_dct_s_2_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw_dct/uvw_lam1_dct_s_2_v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw_dct/uvw_lam1_dct_s_2_u+v_26.56.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw_dct/uvw_lam1_dct_s_2_f-u-v_n_25.jpg}
    \end{minipage}
    }

    \subfigure[Model \eqref{uvw} with Bm3d $u$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw_dct/uvw_lam3_bm3d_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw_dct/uvw_lam3_bm3d_v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw_dct/uvw_lam3_bm3d_u+v_28.6.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_2/uvw_dct/uvw_lam3_bm3d_f-u-v_n_23.jpg}
    \end{minipage}
    }
    \caption{Results using the ROF model, the KR-$L^2$-TV \eqref{kr_new_rel}, the model \eqref{uvw}, the model \eqref{uvw} where $\|v\|_{B_{1,1}^1}$ is replaced by $\|\mathcal{D}v\|$, for $\alpha=100, \lambda=1, \delta=2\sigma$, and the model \eqref{uvw} where \eqref{subw} is replaced by Bm3d.}
    \label{Fig:bar_2_uvw_dct}
\end{figure}





==> KR_denoising/Experiment/grayscale/uvw_dct.tex <==
We propose to replace $\|v\|_{B_{1,1}^1}$ in \eqref{uvw} by $\|\mathcal{D}v\|$ and show the results in Figure \ref{Fig:barbara_dct}.
\begin{figure}
    \centering
    \subfigure[Model \eqref{uvw} with DCT $u$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/uvw_dct/uvw_lam2_dct_32_s_2_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/uvw_dct/uvw_lam2_dct_32_s_2_v.jpg}
    \end{minipage}
    }
    
    \subfigure[$u+v$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/uvw_dct/uvw_lam2_dct_32_s_2_u+v_26.8.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.3\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/uvw_dct/uvw_lam2_dct_32_s_2_f-u-v_n_51.jpg}
    \end{minipage}
    }
    
    \caption{Results using the model \eqref{uvw} where $\|v\|_{B_{1,1}^1}$ is replaced by $\|\mathcal{D}v\|$, for $\alpha=100, \lambda=2, \delta=2\sigma$.}
    \label{Fig:barbara_dct}
\end{figure}


\begin{figure}
    \centering
    \subfigure[Model \eqref{uvw} $u$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/uvw_dct/uvw_lam1_dct_s_2_u.jpg}
    \end{minipage}
    }
    \subfigure[$v+100/25$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/uvw_dct/uvw_lam1_dct_s_2_v.jpg}
    \end{minipage}
    }
    \subfigure[$u+v$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/uvw_dct/uvw_lam1_dct_s_2_u+v_25.2.jpg}
    \end{minipage}
    }
    \subfigure[$f-u-v+100/255$]{
        \begin{minipage}{0.23\linewidth}
        %\caption{FS-TV}
        \centering
        \includegraphics[width=\linewidth]{KR_denoising/figure/new_model/bar_25/barbara_1/uvw_dct/uvw_lam1_dct_s_2_f-u-v_n_25.jpg}
    \end{minipage}
    }
    
    \caption{Results using the model \eqref{uvw} where $\|v\|_{B_{1,1}^1}$ is replaced by $\|\mathcal{D}v\|$, for $\alpha=100, \lambda=1, \delta=2\sigma$.}
    \label{Fig:bar_1_uvw_dct}
\end{figure}
